Histogram Approaches for Imbalanced Data Streams Regression

Imbalanced domains pose a significant challenge in real-world predictive analytics, particularly in the context of regression. While existing research has primarily focused on batch learning from static datasets, limited attention has been given to imbalanced regression in online learning scenarios. Intending to address this gap, in prior work, we proposed sampling strategies based on Chebyshevs inequality as the first methodologies designed explicitly for data streams. However, these approaches operated under the restrictive assumption that rare instances exclusively reside at distribution extremes. This study introduces histogram-based sampling strategies to overcome this constraint, proposing flexible solutions for imbalanced regression in evolving data streams. The proposed techniques -- Histogram-based Undersampling (HistUS) and Histogram-based Oversampling (HistOS) -- employ incremental online histograms to dynamically detect and prioritize rare instances across arbitrary regions of the target distribution to improve predictions in the rare cases. Comprehensive experiments on synthetic and real-world benchmarks demonstrate that HistUS and HistOS substantially improve rare-case prediction accuracy, outperforming baseline models while maintaining competitiveness with Chebyshev-based approaches.

==> Chapters/Sec2-Related-Work/Imbalanced_Regression_old.tex <==
The first challenge %mentioned in the introduction
%is 
resides in
the identification of rare instances. Contrary to classification problems where the minority class of interest is typically well defined, in regression that definition of what are the rare relevant values is more complex by the continuous nature of the target variable.
To tackle the second challenge, which is the tendency of models to bias their predictions toward frequent target values, the existing approaches can be broadly categorized into data-level, algorithm-level, and hybrid techniques. Extensive research has explored imbalanced learning, with \emph{data-level} approaches widely adopted in classification and regression tasks~\cite{hoens2013imbalanced}. These methods modify the dataset rather than the learning algorithm, making them model-agnostic and preserving interpretability~\cite{branco2019pre}.
Among them, sampling techniques are the most common, where overersampling replicates rare instances to enhance their representation~\citep{batista2004study}, and undersampling reduces frequent instances to mitigate bias~\citep{kubat1997addressing}. Some methods combine both strategies to achieve a balanced dataset without excessive data inflation~\citep{RN91}

\begin{comment}

Researchers have developed three principal strategies for imbalanced regression to address this challenge. Kernel Density Estimation (KDE) approaches like \emph{DenseWeight} \citep{steininger2021density} and \emph{WSMOTER} \cite{camacho2024wsmoter} quantify instance rarity through probability density functions, automatically weighting low-density regions without distributional assumptions. Relevance-based methods, exemplified by \citet{ritathesis2011}'s boxplot-derived functions, the SmoteR framework \citep{torgo2013smote}, REBAGG~\cite{pmlr-v94-branco18a}, SMOTEBoost~\cite{moniz2018smoteboost} and G-SMOTE-R ~\cite{camacho2022geometric}, employ piecewise mappings that assign importance scores based on statistical dispersion measures or domain knowledge. The third strategy combines these concepts through distribution-aware binning techniques like \emph{Relevance-based Stratification} \citep{branco2019pre}, which partitions the target space into regions of varying importance. 
\end{comment}
\begin{comment}
To tackle the second challenge, which is the tendency of models to bias their predictions toward frequent target values, the existing approaches can be broadly categorized into data-level, algorithm-level, and hybrid techniques. Extensive research has explored imbalanced learning, with \emph{data-level} approaches widely adopted in classification and regression tasks~\cite{hoens2013imbalanced}. These methods modify the dataset rather than the learning algorithm, making them model-agnostic and preserving interpretability~\cite{branco2019pre}. 

\end{comment}

\begin{comment}
    
Among them, sampling techniques are the most common, where overersampling replicates rare instances to enhance their representation~\citep{batista2004study}, and undersampling reduces frequent instances to mitigate bias~\citep{kubat1997addressing}. Some methods combine both strategies to achieve a balanced dataset without excessive data inflation~\citep{RN91}. 
\end{comment}
A well-known data-level approach is the Synthetic Minority overersampling Technique (SMOTE) \citep{RN91}, designed initially to address class imbalance in classification tasks. Several extensions have been proposed to adapt SMOTE for regression tasks. SMOTER \citep{torgo2013smote} generates synthetic instances to improve the representation of rare cases using relevance-based methods grounded on boxplot-derived functions \citet{ritathesis2011}.
Further extensions include SMOGN \citep{branco2017smogn} that refines the synthetic instance generation process,
%Further extensions, such as 
DistSMOGN \citep{song2022distsmogn} that enables large-scale applications using distributed computing frameworks,
G-SMOTE-R \citep{camacho2022geometric} and WSMOTER \citep{camacho2024wsmoter} that introduce variations tailored to different regression challenges.
Other methods that are not inspired by SMOTE have also been developed, such as ROGN~\cite{branco2019pre}, which combines random overersampling with Gaussian noise injection, and WERCS~\cite{branco2019pre}, which assigns weights to instances and applies a weighted combination of over- and undersampling.


\begin{comment}
While data-level methods provide practical solutions, \emph{algorithm-level} techniques—commonly referred to as cost-sensitive learning—modify the learning process itself by assigning higher penalties to errors on rare instances, ensuring these cases receive greater focus during training~\cite{fernandez2018cost}. Sample weighting strategies, such as DenseWeight and DenseLoss \citep{steininger2021density}, integrate loss-based adaptations to amplify the impact of rare values. Other approaches modify tree-based models to prioritize rare instances, such as the regression tree algorithm proposed by \citet{torgo2003predicting}, which replaces the least squares splitting criterion with an F-measure-based approach to enhance rare extreme value prediction. Kernel density estimation techniques have also been used to smooth label and feature distributions, as seen in LDS and FDS~\cite{yang2021delving}.

\emph{Hybrid techniques} combine data-level and algorithm-level approaches to enhance learning from imbalanced datasets. Ensemble learning strategies such as REBAGG~\citep{pmlr-v94-branco18a} integrate resampling with bagging to balance rare and frequent cases while boosting techniques like SMOTEBoost \citep{moniz2018smoteboost} iteratively generate synthetic instances and adjust sample weights to refine model focus on difficult cases. \citet{huang2022boosting} proposed a hybrid strategy incorporating KDE-based rarity detection with conditional variational autoencoders (CVAE) to generate synthetic samples for boosting-based learning. In contrast, \citet{orhobor2023imbalanced} introduced an ensemble approach that integrates classification and regression to improve prediction on rare values.
\end{comment}


==> Tables/left_OS_phi_8_.tex <==
puma32H & 0.04 $\pm$ 0.0 & $\triangleright$ & \bftab 0.03 $\pm$ 0.0 & 0.04 $\pm$ 0.01 & $\triangleright$ & \bftab 0.02 $\pm$ 0.0 & 0.04 $\pm$ 0.0 & $\triangleright$ & \bftab 0.03 $\pm$ 0.01 & 0.04 $\pm$ 0.0 & $\triangleright$ & \bftab 0.03 $\pm$ 0.01 \\
cpusum & 3.32 $\pm$ 0.11 & $\triangleright$ & \bftab 1.33 $\pm$ 0.02 & 2.88 $\pm$ 0.17 & $\triangleright$ & \bftab 1.3 $\pm$ 0.01 & 6.77 $\pm$ 1.19 & $\triangleright$ & \bftab 2.21 $\pm$ 0.3 & 7.29 $\pm$ 0.3 & $\triangleright$ & \bftab 2.35 $\pm$ 0.07 \\
elevator & 0.13 $\pm$ 0.06 & & \bftab 0.11 $\pm$ 0.09 & \bftab 0.15 $\pm$ 0.03 & $\triangleleft$ & $16\times10^2$ $\pm$ $11\times10^2$ & \bftab 0.13 $\pm$ 0.01 & $\triangleleft$ & $17\times10^2$ $\pm$ 106.2 & \bftab 0.11 $\pm$ 0.0 & $\triangleleft$ & $14\times10^2$ $\pm$ 64.83 \\
bike & 9.93 $\pm$ 0.9 & $\triangleright$ & \bftab 7.15 $\pm$ 1.3 & 46.33 $\pm$ 6.77 & & \bftab 44.92 $\pm$ 6.56 & 223.01 $\pm$ 41.55 & $\triangleright$ & \bftab 144.35 $\pm$ 24.15 & 240.42 $\pm$ 10.54 & $\triangleright$ & \bftab 153.22 $\pm$ 6.71 \\
energy & 230.12 $\pm$ 3.38 & $\triangleright$ & \bftab 187.25 $\pm$ 2.09 & 235.91 $\pm$ 0.6 & $\triangleright$ & \bftab 192.46 $\pm$ 0.73 & 241.68 $\pm$ 2.39 & $\triangleright$ & \bftab 194.53 $\pm$ 0.96 & 241.88 $\pm$ 1.27 & $\triangleright$ & \bftab 194.71 $\pm$ 0.52 \\
calhousing & $14\times10^4$ $\pm$ $19\times10^2$ & $\triangleright$ & \bftab $10\times10^4$ $\pm$ $18\times10^2$ & $13\times10^4$ $\pm$ $22\times10^2$ & $\triangleright$ & \bftab $10\times10^4$ $\pm$ $12\times10^2$ & $17\times10^4$ $\pm$ $13\times10^3$ & $\triangleright$ & \bftab $11\times10^4$ $\pm$ $50\times10^2$ & $18\times10^4$ $\pm$ $35\times10^2$ & $\triangleright$ & \bftab $11\times10^4$ $\pm$ $11\times10^2$ \\
gasemission & 19.19 $\pm$ 0.17 & $\triangleright$ & \bftab 12.94 $\pm$ 0.14 & 17.91 $\pm$ 0.63 & $\triangleright$ & \bftab 12.36 $\pm$ 0.27 & 20.86 $\pm$ 1.78 & $\triangleright$ & \bftab 14.32 $\pm$ 1.09 & 21.6 $\pm$ 0.64 & $\triangleright$ & \bftab 14.9 $\pm$ 0.32 \\
mv & 5.62 $\pm$ 0.17 & $\triangleright$ & \bftab 0.74 $\pm$ 0.02 & 4.37 $\pm$ 0.37 & $\triangleright$ & \bftab 0.61 $\pm$ 0.05 & 5.93 $\pm$ 0.48 & $\triangleright$ & \bftab 0.93 $\pm$ 0.09 & 5.77 $\pm$ 0.27 & $\triangleright$ & \bftab 0.86 $\pm$ 0.3 \\
fried & 3.88 $\pm$ 0.02 & $\triangleright$ & \bftab 3.64 $\pm$ 0.02 & 3.42 $\pm$ 0.16 & $\triangleright$ & \bftab 3.15 $\pm$ 0.18 & 5.82 $\pm$ 0.81 & $\triangleright$ & \bftab 4.01 $\pm$ 0.37 & 6.23 $\pm$ 0.18 & $\triangleright$ & \bftab 4.19 $\pm$ 0.09 \\
polution & 194.58 $\pm$ 2.49 & $\triangleright$ & \bftab 130.29 $\pm$ 2.19 & 177.34 $\pm$ 5.61 & $\triangleright$ & \bftab 120.81 $\pm$ 2.59 & 189.49 $\pm$ 6.12 & $\triangleright$ & \bftab 128.25 $\pm$ 3.32 & 191.92 $\pm$ 1.5 & $\triangleright$ & \bftab 129.39 $\pm$ 0.78 \\
car price & $35\times10^3$ $\pm$ 384.03 & $\triangleright$ & \bftab $25\times10^3$ $\pm$ 373.09 & $33\times10^3$ $\pm$ 575.38 & & \bftab $31\times10^3$ $\pm$ $44\times10^2$ & $34\times10^3$ $\pm$ 393.88 & & \bftab $33\times10^3$ $\pm$ 654.55 & $33\times10^3$ $\pm$ 311.73 & $\triangleright$ & \bftab $31\times10^3$ $\pm$ 589.8 \\
query & 451.03 $\pm$ 6.02 & $\triangleright$ & \bftab 270.98 $\pm$ 3.19 & 366.3 $\pm$ 28.72 & $\triangleright$ & \bftab 223.04 $\pm$ 16.52 & 403.45 $\pm$ 23.28 & $\triangleright$ & \bftab 246.39 $\pm$ 13.93 & 420.29 $\pm$ 3.09 & $\triangleright$ & \bftab 254.43 $\pm$ 3.41 \\
GPU & 600.71 $\pm$ 3.41 & $\triangleright$ & \bftab 406.95 $\pm$ 2.31 & 484.93 $\pm$ 58.26 & $\triangleright$ & \bftab 329.3 $\pm$ 39.03 & 553.89 $\pm$ 65.81 & $\triangleright$ & \bftab 392.4 $\pm$ 52.03 & 588.3 $\pm$ 18.67 & $\triangleright$ & \bftab 423.71 $\pm$ 12.65 \\
3d & 44.01 $\pm$ 0.06 & $\triangleright$ & \bftab 24.93 $\pm$ 0.07 & 32.49 $\pm$ 10.73 & $\triangleright$ & \bftab 18.89 $\pm$ 5.57 & 42.21 $\pm$ 1.89 & $\triangleright$ & \bftab 26.38 $\pm$ 1.18 & 40.41 $\pm$ 1.72 & $\triangleright$ & \bftab 24.97 $\pm$ 1.24 \\


==> Tables/left_US_phi_8_.tex <==
puma32H & 0.04 $\pm$ 0.0 & $\triangleright$ & \bftab 0.02 $\pm$ 0.0 & 0.04 $\pm$ 0.01 & $\triangleright$ & \bftab 0.02 $\pm$ 0.0 & 0.04 $\pm$ 0.0 & $\triangleright$ & \bftab 0.02 $\pm$ 0.0 & 0.04 $\pm$ 0.0 & $\triangleright$ & \bftab 0.02 $\pm$ 0.0 \\
cpusum & \bftab 3.32 $\pm$ 0.11 & $\triangleleft$ & 91.71 $\pm$ 0.1 & \bftab 2.88 $\pm$ 0.17 & $\triangleleft$ & 91.61 $\pm$ 0.04 & \bftab 6.77 $\pm$ 1.19 & $\triangleleft$ & 91.58 $\pm$ 0.02 & \bftab 7.29 $\pm$ 0.3 & $\triangleleft$ & 91.56 $\pm$ 0.02 \\
elevator & 0.13 $\pm$ 0.06 & & \bftab 0.08 $\pm$ 0.06 & 0.15 $\pm$ 0.03 & $\triangleright$ & \bftab 0.04 $\pm$ 0.01 & 0.13 $\pm$ 0.01 & $\triangleright$ & \bftab 0.03 $\pm$ 0.0 & 0.11 $\pm$ 0.0 & $\triangleright$ & \bftab 0.04 $\pm$ 0.01 \\
bike & \bftab 9.93 $\pm$ 0.9 & $\triangleleft$ & 13.2 $\pm$ 1.74 & \bftab 46.33 $\pm$ 6.77 & $\triangleleft$ & 69.84 $\pm$ 8.59 & 223.01 $\pm$ 41.55 & $\triangleright$ & \bftab 123.97 $\pm$ 13.91 & 240.42 $\pm$ 10.54 & $\triangleright$ & \bftab 125.46 $\pm$ 5.46 \\
energy & 230.12 $\pm$ 3.38 & $\triangleright$ & \bftab 167.48 $\pm$ 1.79 & 235.91 $\pm$ 0.6 & $\triangleright$ & \bftab 181.07 $\pm$ 3.28 & 241.68 $\pm$ 2.39 & $\triangleright$ & \bftab 179.1 $\pm$ 1.94 & 241.88 $\pm$ 1.27 & $\triangleright$ & \bftab 175.09 $\pm$ 0.85 \\
calhousing & $14\times10^4$ $\pm$ $19\times10^2$ & $\triangleright$ & \bftab $86\times10^3$ $\pm$ $10\times10^2$ & $13\times10^4$ $\pm$ $22\times10^2$ & $\triangleright$ & \bftab $86\times10^3$ $\pm$ 467.64 & $17\times10^4$ $\pm$ $13\times10^3$ & $\triangleright$ & \bftab $90\times10^3$ $\pm$ $16\times10^2$ & $18\times10^4$ $\pm$ $35\times10^2$ & $\triangleright$ & \bftab $91\times10^3$ $\pm$ 555.19 \\
gasemission & 19.19 $\pm$ 0.17 & $\triangleright$ & \bftab 11.5 $\pm$ 0.14 & 17.91 $\pm$ 0.63 & $\triangleright$ & \bftab 11.58 $\pm$ 0.09 & 20.86 $\pm$ 1.78 & $\triangleright$ & \bftab 12.89 $\pm$ 0.63 & 21.6 $\pm$ 0.64 & $\triangleright$ & \bftab 13.22 $\pm$ 0.19 \\
mv & 5.62 $\pm$ 0.17 & $\triangleright$ & \bftab 0.64 $\pm$ 0.1 & 4.37 $\pm$ 0.37 & $\triangleright$ & \bftab 1.13 $\pm$ 0.1 & 5.93 $\pm$ 0.48 & $\triangleright$ & \bftab 1.11 $\pm$ 0.04 & 5.77 $\pm$ 0.27 & $\triangleright$ & \bftab 0.91 $\pm$ 0.32 \\
fried & 3.88 $\pm$ 0.02 & $\triangleright$ & \bftab 2.93 $\pm$ 0.03 & 3.42 $\pm$ 0.16 & $\triangleright$ & \bftab 2.73 $\pm$ 0.06 & 5.82 $\pm$ 0.81 & $\triangleright$ & \bftab 3.38 $\pm$ 0.25 & 6.23 $\pm$ 0.18 & $\triangleright$ & \bftab 3.52 $\pm$ 0.05 \\
polution & 194.58 $\pm$ 2.49 & $\triangleright$ & \bftab 105.82 $\pm$ 3.04 & 177.34 $\pm$ 5.61 & $\triangleright$ & \bftab 102.08 $\pm$ 0.98 & 189.49 $\pm$ 6.12 & $\triangleright$ & \bftab 106.82 $\pm$ 1.78 & 191.92 $\pm$ 1.5 & $\triangleright$ & \bftab 107.96 $\pm$ 0.16 \\
car price & $35\times10^3$ $\pm$ 384.03 & $\triangleright$ & \bftab $29\times10^3$ $\pm$ $28\times10^2$ & $33\times10^3$ $\pm$ 575.38 & $\triangleright$ & \bftab $30\times10^3$ $\pm$ $12\times10^2$ & $34\times10^3$ $\pm$ 393.88 & $\triangleright$ & \bftab $29\times10^3$ $\pm$ 545.84 & $33\times10^3$ $\pm$ 311.73 & $\triangleright$ & \bftab $28\times10^3$ $\pm$ 485.23 \\
query & 451.03 $\pm$ 6.02 & $\triangleright$ & \bftab 228.16 $\pm$ 2.82 & 366.3 $\pm$ 28.72 & $\triangleright$ & \bftab 193.52 $\pm$ 11.63 & 403.45 $\pm$ 23.28 & $\triangleright$ & \bftab 211.52 $\pm$ 10.29 & 420.29 $\pm$ 3.09 & $\triangleright$ & \bftab 217.15 $\pm$ 1.99 \\
GPU & 600.71 $\pm$ 3.41 & $\triangleright$ & \bftab 385.25 $\pm$ 1.8 & 484.93 $\pm$ 58.26 & $\triangleright$ & \bftab 327.16 $\pm$ 29.18 & 553.89 $\pm$ 65.81 & $\triangleright$ & \bftab 374.1 $\pm$ 38.71 & 588.3 $\pm$ 18.67 & $\triangleright$ & \bftab 399.33 $\pm$ 8.63 \\
3d & 44.01 $\pm$ 0.06 & $\triangleright$ & \bftab 19.0 $\pm$ 0.07 & 32.49 $\pm$ 10.73 & $\triangleright$ & \bftab 15.86 $\pm$ 2.62 & 42.21 $\pm$ 1.89 & $\triangleright$ & \bftab 20.39 $\pm$ 0.73 & 40.41 $\pm$ 1.72 & $\triangleright$ & \bftab 19.5 $\pm$ 0.7 \\


==> Tables/normal_Over.tex <==
puma32H & 0.020 $\pm$ 0.000 &  & 0.020 $\pm$ 0.000 & 0.030 $\pm$ 0.000 &  & 0.030 $\pm$ 0.000 & 0.020 $\pm$ 0.000 & $\triangleright$ & \bftab 0.014 $\pm$ 0.000 & 0.030 $\pm$ 0.000 &  & 0.030 $\pm$ 0.000 \\ 
cpusum & 7.991 $\pm$ 0.221 &  & \bftab 6.888 $\pm$ 5.300 & \bftab 10.83 $\pm$ 0.171 & $\triangleleft$ & 11.42 $\pm$ 0.056 & 6.894 $\pm$ 0.064 &  & \bftab 6.746 $\pm$ 0.226 & \bftab 18.99 $\pm$ 0.107 & $\triangleleft$ & 19.99 $\pm$ 0.045 \\ 
mv & \bftab 1.618 $\pm$ 0.025 &  & 1.687 $\pm$ 0.042 & \bftab 4.497 $\pm$ 0.000 & $\triangleleft$ & 4.535 $\pm$ 0.000 & 1.183 $\pm$ 0.012 & $\triangleright$ & \bftab 0.785 $\pm$ 0.003 & \bftab 10.43 $\pm$ 0.001 & $\triangleleft$ & 10.54 $\pm$ 0.000 \\ 
elevator & 0.053 $\pm$ 0.003 &  & \bftab 0.024 $\pm$ 0.001 & \bftab 0.029 $\pm$ 0.001 &  & 0.050 $\pm$ 0.002 & \bftab 0.006 $\pm$ 0.000 &  & 0.026 $\pm$ 0.003 & 0.010 $\pm$ 0.000 &  & 0.010 $\pm$ 0.000 \\ 
energydata-complete & \bftab 97.55 $\pm$ 0.488 & $\triangleleft$ & 108.2 $\pm$ 1.765 & \bftab 95.40 $\pm$ 3.350 & $\triangleleft$ & 104.9 $\pm$ 4.535 & \bftab 104.9 $\pm$ 10.87 & $\triangleleft$ & 114.2 $\pm$ 10.82 & \bftab 102.9 $\pm$ 2.222 & $\triangleleft$ & 109.1 $\pm$ 18.35 \\ 
FriedmanArtificialDomain & \bftab 2.377 $\pm$ 0.001 & $\triangleleft$ & 2.406 $\pm$ 0.001 & \bftab 2.641 $\pm$ 0.000 & $\triangleleft$ & 2.659 $\pm$ 0.000 & 2.198 $\pm$ 0.001 & $\triangleright$ & \bftab 2.035 $\pm$ 0.001 & 4.998 $\pm$ 0.000 &  & 4.998 $\pm$ 0.000 \\ 
california & \bftab 68003 $\pm$ 381 & $\triangleleft$ & 69111 $\pm$ 528 & \bftab 70389 $\pm$ 181 & $\triangleleft$ & 71213 $\pm$ 92971 & \bftab 74753 $\pm$ 2991 &  & 74949 $\pm$ 3997 & \bftab 115 $\pm$ 81585 & $\triangleleft$ & 116 $\pm$ 38747 \\ 
bike & \bftab 4.881 $\pm$ 1.151 &  & 5.269 $\pm$ 1.000 & \bftab 8.195 $\pm$ 1.027 &  & 8.215 $\pm$ 1.451 & 65.01 $\pm$ 14.27 &  & \bftab 62.74 $\pm$ 34.37 & \bftab 181.6 $\pm$ 0.363 & $\triangleleft$ & 184.0 $\pm$ 0.232 \\ 
3d-spatial-network & 14.49 $\pm$ 0.065 &  & \bftab 14.35 $\pm$ 0.012 & \bftab 18.28 $\pm$ 0.000 & $\triangleleft$ & 18.51 $\pm$ 0.001 & 8.650 $\pm$ 0.347 & $\triangleright$ & \bftab 7.540 $\pm$ 0.155 & \bftab 18.62 $\pm$ 0.000 & $\triangleleft$ & 18.82 $\pm$ 0.000 \\ 
Range-Queries-Aggregates & 118.0 $\pm$ 16.06 & $\triangleright$ & \bftab 113.0 $\pm$ 15.60 & \bftab 133.8 $\pm$ 0.135 & $\triangleleft$ & 134.9 $\pm$ 0.133 & 63.91 $\pm$ 1.780 & $\triangleright$ & \bftab 59.50 $\pm$ 2.514 & \bftab 268.7 $\pm$ 0.114 & $\triangleleft$ & 268.7 $\pm$ 0.114 \\ 
pp-gas-emission & 6.605 $\pm$ 0.014 & $\triangleright$ & \bftab 6.515 $\pm$ 0.006 & \bftab 8.033 $\pm$ 0.001 & $\triangleleft$ & 8.153 $\pm$ 0.002 & 7.930 $\pm$ 0.032 & $\triangleright$ & \bftab 7.533 $\pm$ 0.019 & \bftab 11.68 $\pm$ 0.002 & $\triangleleft$ & 11.74 $\pm$ 0.002 \\ 
GPU-Kernel-Performance & \bftab 199.4 $\pm$ 66.95 & $\triangleleft$ & 208.3 $\pm$ 11.20 & \bftab 284.5 $\pm$ 2.086 & $\triangleleft$ & 322.2 $\pm$ 4.737 & \bftab 43.44 $\pm$ 4.244 &  & 47.36 $\pm$ 107.0 & \bftab 368.4 $\pm$ 0.929 & $\triangleleft$ & 387.2 $\pm$ 0.322 \\ 
polution & \bftab 74.56 $\pm$ 1.188 & $\triangleleft$ & 78.46 $\pm$ 0.710 & \bftab 79.55 $\pm$ 0.138 & $\triangleleft$ & 83.16 $\pm$ 0.212 & \bftab 68.55 $\pm$ 0.904 & $\triangleleft$ & 71.50 $\pm$ 7.755 & \bftab 91.96 $\pm$ 0.078 & $\triangleleft$ & 94.51 $\pm$ 0.060


==> Tables/normal_Over_OLD.tex <==
puma32H & 0.022 $\pm$ 0.000 &  & \bftab 0.020 $\pm$ 0.000 & 0.030 $\pm$ 0.000 &  & 0.030 $\pm$ 0.000 & 0.020 $\pm$ 0.000 &  & \bftab 0.019 $\pm$ 0.000 & 0.030 $\pm$ 0.000 &  & 0.030 $\pm$ 0.000 \\ 
cpusum & \bftab 7.287 $\pm$ 0.402 &  & 7.378 $\pm$ 3.231 & \bftab 10.66 $\pm$ 1.139 &  & 10.96 $\pm$ 0.494 & 8.789 $\pm$ 0.747 & $\triangleright$ & \bftab 6.398 $\pm$ 0.070 & \bftab 18.97 $\pm$ 0.663 & $\triangleleft$ & 20.10 $\pm$ 0.318 \\ 
mv & \bftab 1.510 $\pm$ 0.121 &  & 1.743 $\pm$ 0.264 & \bftab 4.489 $\pm$ 0.014 & $\triangleleft$ & 4.596 $\pm$ 0.019 & 0.975 $\pm$ 0.011 & $\triangleright$ & \bftab 0.569 $\pm$ 0.003 & \bftab 10.34 $\pm$ 0.020 & $\triangleleft$ & 10.85 $\pm$ 0.012 \\ 
elevator & 0.069 $\pm$ 0.012 &  & \bftab 0.015 $\pm$ 0.001 & \bftab 0.004 $\pm$ 0.000 &  & 0.044 $\pm$ 0.008 & \bftab 0.023 $\pm$ 0.004 & $\triangleleft$ & 3.718 $\pm$ 95.43 & 0.010 $\pm$ 0.000 &  & 0.010 $\pm$ 0.000 \\ 
energydata-complete & \bftab 93.75 $\pm$ 8.036 & $\triangleleft$ & 103.3 $\pm$ 10.14 & \bftab 93.68 $\pm$ 11.71 & $\triangleleft$ & 102.2 $\pm$ 15.91 & \bftab 104.0 $\pm$ 10.61 & $\triangleleft$ & 111.6 $\pm$ 17.69 & \bftab 101.1 $\pm$ 4.747 & $\triangleleft$ & 110.1 $\pm$ 2.654 \\ 
FriedmanArtificialDomain & \bftab 2.408 $\pm$ 0.004 &  & 2.451 $\pm$ 0.004 & \bftab 2.655 $\pm$ 0.003 & $\triangleleft$ & 2.693 $\pm$ 0.003 & 2.142 $\pm$ 0.001 & $\triangleright$ & \bftab 2.058 $\pm$ 0.002 & 4.987 $\pm$ 0.002 &  & 4.987 $\pm$ 0.002 \\ 
california & \bftab 67046 $\pm$ 7482 &  & 68163 $\pm$ 2812 & \bftab 69902 $\pm$ 1688 & $\triangleleft$ & 71088 $\pm$ 1937 & 76531 $\pm$ 50443 &  & \bftab 76261 $\pm$ 48846 & \bftab 115 $\pm$ 2181 & $\triangleleft$ & 117 $\pm$ 1324 \\ 
bike & \bftab 4.379 $\pm$ 0.791 &  & 6.005 $\pm$ 7.214 & 6.804 $\pm$ 5.023 &  & \bftab 6.527 $\pm$ 4.960 & 62.82 $\pm$ 21.52 & $\triangleright$ & \bftab 57.25 $\pm$ 19.79 & \bftab 182.9 $\pm$ 12.77 & $\triangleleft$ & 193.3 $\pm$ 8.073 \\ 
3d-spatial-network & \bftab 14.24 $\pm$ 0.333 &  & 14.47 $\pm$ 0.193 & \bftab 18.28 $\pm$ 0.031 & $\triangleleft$ & 19.07 $\pm$ 0.022 & 7.670 $\pm$ 0.101 & $\triangleright$ & \bftab 6.873 $\pm$ 0.194 & \bftab 18.52 $\pm$ 0.022 & $\triangleleft$ & 19.30 $\pm$ 0.012 \\ 
Range-Queries-Aggregates & 116.9 $\pm$ 17.03 & $\triangleright$ & \bftab 111.8 $\pm$ 43.08 & \bftab 132.7 $\pm$ 6.010 & $\triangleleft$ & 133.1 $\pm$ 5.920 & 61.28 $\pm$ 13.38 & $\triangleright$ & \bftab 53.49 $\pm$ 9.888 & \bftab 268.6 $\pm$ 1.358 & $\triangleleft$ & 268.8 $\pm$ 1.267 \\ 
pp-gas-emission & \bftab 6.558 $\pm$ 0.082 &  & 6.581 $\pm$ 0.074 & \bftab 8.049 $\pm$ 0.022 & $\triangleleft$ & 8.249 $\pm$ 0.020 & 7.446 $\pm$ 0.013 &  & \bftab 7.353 $\pm$ 0.065 & \bftab 11.65 $\pm$ 0.022 & $\triangleleft$ & 11.83 $\pm$ 0.020 \\ 
GPU-Kernel-Performance & 198.8 $\pm$ 123.1 &  & \bftab 191.6 $\pm$ 124.7 & \bftab 283.0 $\pm$ 63.45 & $\triangleleft$ & 288.0 $\pm$ 49.06 & \bftab 38.14 $\pm$ 12.22 &  & 38.38 $\pm$ 82.33 & \bftab 369.6 $\pm$ 10.89 & $\triangleleft$ & 381.2 $\pm$ 8.695 \\ 
polution & \bftab 74.11 $\pm$ 5.493 & $\triangleleft$ & 78.97 $\pm$ 3.458 & \bftab 79.94 $\pm$ 1.227 & $\triangleleft$ & 84.25 $\pm$ 1.195 & \bftab 67.51 $\pm$ 5.513 & $\triangleleft$ & 70.10 $\pm$ 3.771 & \bftab 92.46 $\pm$ 2.127 & $\triangleleft$ & 98.06 $\pm$ 1.103  


==> Tables/normal_Un_OS.tex <==
puma32H & 0.02 $\pm$ 0.00 &  & \bftab 0.02 $\pm$ 0.00 & 0.03 $\pm$ 0.00 &  & 0.03 $\pm$ 0.00 & 0.03 $\pm$ 0.00 & $\triangleright$ & \bftab 0.02 $\pm$ 0.00 & 0.03 $\pm$ 0.00 &  & 0.03 $\pm$ 0.00 \\ 
cpusum & 10.89 $\pm$ 3.01 & $\triangleright$ & \bftab 7.19 $\pm$ 4.77 & 12.04 $\pm$ 0.51 &  & \bftab 11.84 $\pm$ 0.42 & 14.27 $\pm$ 0.37 & $\triangleright$ & \bftab 7.50 $\pm$ 0.76 & \bftab 19.78 $\pm$ 0.10 & $\triangleleft$ & 20.08 $\pm$ 0.11 \\ 
mv & 1.66 $\pm$ 0.06 &  & \bftab 1.55 $\pm$ 0.02 & \bftab 4.59 $\pm$ 0.00 & $\triangleleft$ & 4.62 $\pm$ 0.00 & 1.88 $\pm$ 0.02 & $\triangleright$ & \bftab 0.75 $\pm$ 0.00 & \bftab 10.70 $\pm$ 0.00 & $\triangleleft$ & 10.87 $\pm$ 0.00 \\ 
elevator & 0.04 $\pm$ 0.00 &  & \bftab 0.03 $\pm$ 0.00 & \bftab 0.02 $\pm$ 0.00 &  & 0.04 $\pm$ 0.00 & \bftab 0.01 $\pm$ 0.00 & $\triangleleft$ & 4e+06 $\pm$ 2e+14 & 0.01 $\pm$ 0.00 &  & 0.01 $\pm$ 0.00 \\ 
energydata-complete & \bftab 102.81 $\pm$ 2.16 & $\triangleleft$ & 108.05 $\pm$ 1.65 & \bftab 102.75 $\pm$ 0.70 & $\triangleleft$ & 105.89 $\pm$ 1.19 & 122.51 $\pm$ 2.76 & $\triangleright$ & \bftab 118.72 $\pm$ 12.68 & \bftab 108.15 $\pm$ 0.44 & $\triangleleft$ & 111.43 $\pm$ 0.39 \\ 
FriedmanArtificialDomain & 2.55 $\pm$ 0.00 & $\triangleright$ & \bftab 2.43 $\pm$ 0.00 & \bftab 2.68 $\pm$ 0.00 &  & 2.68 $\pm$ 0.00 & 2.57 $\pm$ 0.01 & $\triangleright$ & \bftab 2.17 $\pm$ 0.00 & 5.00 $\pm$ 0.00 &  & \bftab 5.00 $\pm$ 0.00 \\ 
california & 7e+04 $\pm$ 7e+05 &  & \bftab 7e+04 $\pm$ 8e+05 & 7e+04 $\pm$ 2e+06 & $\triangleright$ & \bftab 7e+04 $\pm$ 6e+05 & 8e+04 $\pm$ 1e+07 & $\triangleright$ & \bftab 8e+04 $\pm$ 9e+06 & \bftab 1e+05 $\pm$ 3e+05 & $\triangleleft$ & 1e+05 $\pm$ 3e+05 \\ 
bike & \bftab 5.28 $\pm$ 0.98 & $\triangleleft$ & 6.95 $\pm$ 2.34 & 10.26 $\pm$ 0.43 & $\triangleright$ & \bftab 7.21 $\pm$ 12.27 & 87.92 $\pm$ 6.30 & $\triangleright$ & \bftab 66.62 $\pm$ 24.76 & \bftab 188.35 $\pm$ 0.65 & $\triangleleft$ & 191.97 $\pm$ 0.88 \\ 
3d-spatial-network & 15.10 $\pm$ 0.13 & $\triangleright$ & \bftab 14.69 $\pm$ 0.02 & \bftab 18.69 $\pm$ 0.00 & $\triangleleft$ & 19.08 $\pm$ 0.00 & 9.30 $\pm$ 0.06 & $\triangleright$ & \bftab 7.70 $\pm$ 0.08 & \bftab 19.00 $\pm$ 0.00 & $\triangleleft$ & 19.38 $\pm$ 0.00 \\ 
Range-Queries-Aggregates & 117.86 $\pm$ 28.96 &  & \bftab 115.34 $\pm$ 22.52 & \bftab 134.22 $\pm$ 0.17 & $\triangleleft$ & 134.47 $\pm$ 0.15 & 68.94 $\pm$ 2.75 & $\triangleright$ & \bftab 60.26 $\pm$ 3.18 & 269.00 $\pm$ 0.04 & $\triangleright$ & \bftab 268.97 $\pm$ 0.03 \\ 
pp-gas-emission & 6.82 $\pm$ 0.01 &  & \bftab 6.75 $\pm$ 0.03 & 8.44 $\pm$ 0.00 & $\triangleright$ & \bftab 8.33 $\pm$ 0.00 & 9.57 $\pm$ 0.03 & $\triangleright$ & \bftab 8.08 $\pm$ 0.03 & \bftab 11.80 $\pm$ 0.00 & $\triangleleft$ & 11.88 $\pm$ 0.00 \\ 
GPU-Kernel-Performance & 203.95 $\pm$ 8.95 & $\triangleright$ & \bftab 193.96 $\pm$ 21.52 & \bftab 286.48 $\pm$ 0.82 & $\triangleleft$ & 289.47 $\pm$ 0.69 & 61.46 $\pm$ 24.39 & $\triangleright$ & \bftab 44.29 $\pm$ 69.58 & \bftab 374.46 $\pm$ 1.29 & $\triangleleft$ & 380.50 $\pm$ 0.94 \\ 
polution & \bftab 78.54 $\pm$ 0.17 &  & 79.10 $\pm$ 1.04 & \bftab 81.49 $\pm$ 2.22 & $\triangleleft$ & 83.13 $\pm$ 3.34 & 75.29 $\pm$ 12.25 &  & \bftab 75.15 $\pm$ 20.40 & \bftab 91.36 $\pm$ 76.51 & $\triangleleft$ & 93.27 $\pm$ 91.06


==> Tables/normal_Under.tex <==
puma32H & \bftab 0.020 $\pm$ 0.000 & $\triangleleft$ & 0.027 $\pm$ 0.000 & 0.030 $\pm$ 0.000 &  & 0.030 $\pm$ 0.000 & \bftab 0.020 $\pm$ 0.000 & $\triangleleft$ & 0.043 $\pm$ 0.000 & 0.030 $\pm$ 0.000 &  & 0.030 $\pm$ 0.000 \\ 
cpusum & \bftab 7.991 $\pm$ 0.221 & $\triangleleft$ & 25.87 $\pm$ 59.21 & \bftab 10.83 $\pm$ 0.171 & $\triangleleft$ & 18.18 $\pm$ 3.953 & \bftab 6.894 $\pm$ 0.064 & $\triangleleft$ & 33.75 $\pm$ 3.848 & \bftab 18.99 $\pm$ 0.107 & $\triangleleft$ & 39.44 $\pm$ 0.192 \\ 
mv & \bftab 1.618 $\pm$ 0.025 & $\triangleleft$ & 2.219 $\pm$ 0.050 & \bftab 4.497 $\pm$ 0.000 & $\triangleleft$ & 4.805 $\pm$ 0.001 & \bftab 1.183 $\pm$ 0.012 & $\triangleleft$ & 3.687 $\pm$ 0.041 & \bftab 10.43 $\pm$ 0.001 & $\triangleleft$ & 12.85 $\pm$ 0.001 \\ 
elevator & 0.053 $\pm$ 0.003 &  & \bftab 0.022 $\pm$ 0.001 & 0.029 $\pm$ 0.001 &  & \bftab 0.020 $\pm$ 0.000 & \bftab 0.006 $\pm$ 0.000 &  & 0.010 $\pm$ 0.000 & 0.010 $\pm$ 0.000 &  & 0.010 $\pm$ 0.000 \\ 
energydata-complete & \bftab 97.55 $\pm$ 0.488 & $\triangleleft$ & 165.2 $\pm$ 2.981 & \bftab 95.40 $\pm$ 3.350 & $\triangleleft$ & 163.5 $\pm$ 6.284 & \bftab 104.9 $\pm$ 10.87 & $\triangleleft$ & 203.0 $\pm$ 170.6 & \bftab 102.9 $\pm$ 2.222 & $\triangleleft$ & 176.1 $\pm$ 164.9 \\ 
FriedmanArtificialDomain & \bftab 2.377 $\pm$ 0.001 & $\triangleleft$ & 2.726 $\pm$ 0.002 & \bftab 2.641 $\pm$ 0.000 & $\triangleleft$ & 2.776 $\pm$ 0.000 & \bftab 2.198 $\pm$ 0.001 & $\triangleleft$ & 2.936 $\pm$ 0.028 & 4.998 $\pm$ 0.000 &  & 4.998 $\pm$ 0.000 \\ 
california & \bftab 68003 $\pm$ 381 & $\triangleleft$ & 79511 $\pm$ 1995 & \bftab 70389 $\pm$ 181 & $\triangleleft$ & 83108 $\pm$ 10189 & \bftab 74753 $\pm$ 2991 & $\triangleleft$ & 101 $\pm$ 16737 & \bftab 115 $\pm$ 81585 & $\triangleleft$ & 129 $\pm$ 492 \\ 
bike & \bftab 4.881 $\pm$ 1.151 & $\triangleleft$ & 8.056 $\pm$ 4.522 & \bftab 8.195 $\pm$ 1.027 & $\triangleleft$ & 15.74 $\pm$ 3.060 & \bftab 65.01 $\pm$ 14.27 & $\triangleleft$ & 172.7 $\pm$ 206.5 & \bftab 181.6 $\pm$ 0.363 & $\triangleleft$ & 244.2 $\pm$ 1.971 \\ 
3d-spatial-network & \bftab 14.49 $\pm$ 0.065 & $\triangleleft$ & 18.35 $\pm$ 0.593 & \bftab 18.28 $\pm$ 0.000 & $\triangleleft$ & 22.24 $\pm$ 0.002 & \bftab 8.650 $\pm$ 0.347 & $\triangleleft$ & 12.20 $\pm$ 0.166 & \bftab 18.62 $\pm$ 0.000 & $\triangleleft$ & 22.93 $\pm$ 0.002 \\ 
Range-Queries-Aggregates & \bftab 118.0 $\pm$ 16.06 &  & 126.7 $\pm$ 43.31 & \bftab 133.8 $\pm$ 0.135 & $\triangleleft$ & 142.1 $\pm$ 0.237 & \bftab 63.91 $\pm$ 1.780 & $\triangleleft$ & 83.76 $\pm$ 8.555 & \bftab 268.7 $\pm$ 0.114 & $\triangleleft$ & 268.8 $\pm$ 0.121 \\ 
pp-gas-emission & \bftab 6.605 $\pm$ 0.014 & $\triangleleft$ & 7.438 $\pm$ 0.012 & \bftab 8.033 $\pm$ 0.001 & $\triangleleft$ & 9.354 $\pm$ 0.005 & \bftab 7.930 $\pm$ 0.032 & $\triangleleft$ & 11.84 $\pm$ 0.060 & \bftab 11.68 $\pm$ 0.002 & $\triangleleft$ & 12.14 $\pm$ 0.001 \\ 
GPU-Kernel-Performance & \bftab 199.4 $\pm$ 66.95 & $\triangleleft$ & 277.2 $\pm$ 93.60 & \bftab 284.5 $\pm$ 2.086 & $\triangleleft$ & 422.0 $\pm$ 7.345 & \bftab 43.44 $\pm$ 4.244 & $\triangleleft$ & 185.6 $\pm$ 360.9 & \bftab 368.4 $\pm$ 0.929 & $\triangleleft$ & 637.7 $\pm$ 1.918 \\ 
polution & \bftab 74.56 $\pm$ 1.188 & $\triangleleft$ & 109.8 $\pm$ 4.134 & \bftab 79.55 $\pm$ 0.138 & $\triangleleft$ & 111.5 $\pm$ 10.46 & \bftab 68.55 $\pm$ 0.904 & $\triangleleft$ & 106.8 $\pm$ 4.059 & \bftab 91.96 $\pm$ 0.078 & $\triangleleft$ & 132.9 $\pm$ 0.321

==> Tables/normal_Under_OLD.tex <==
puma32H & \bftab 0.022 $\pm$ 0.000 &  & 0.024 $\pm$ 0.000 & 0.030 $\pm$ 0.000 &  & 0.030 $\pm$ 0.000 & \bftab 0.020 $\pm$ 0.000 & $\triangleleft$ & 0.030 $\pm$ 0.000 & 0.030 $\pm$ 0.000 &  & 0.030 $\pm$ 0.000 \\ 
cpusum & \bftab 7.287 $\pm$ 0.402 & $\triangleleft$ & 10.63 $\pm$ 6.259 & \bftab 10.66 $\pm$ 1.139 &  & 11.07 $\pm$ 0.371 & \bftab 8.789 $\pm$ 0.747 & $\triangleleft$ & 13.76 $\pm$ 0.182 & \bftab 18.97 $\pm$ 0.663 & $\triangleleft$ & 19.78 $\pm$ 0.344 \\ 
mv & 1.510 $\pm$ 0.121 &  & \bftab 1.419 $\pm$ 0.060 & \bftab 4.489 $\pm$ 0.014 & $\triangleleft$ & 4.575 $\pm$ 0.019 & \bftab 0.975 $\pm$ 0.011 &  & 1.086 $\pm$ 0.015 & \bftab 10.34 $\pm$ 0.020 & $\triangleleft$ & 10.66 $\pm$ 0.013 \\ 
elevator & \bftab 0.069 $\pm$ 0.012 &  & 0.083 $\pm$ 0.013 & 0.004 $\pm$ 0.000 &  & 0.004 $\pm$ 0.000 & 0.023 $\pm$ 0.004 &  & \bftab 0.006 $\pm$ 0.000 & 0.010 $\pm$ 0.000 &  & 0.010 $\pm$ 0.000 \\ 
energydata-complete & \bftab 93.75 $\pm$ 8.036 & $\triangleleft$ & 98.43 $\pm$ 6.211 & \bftab 93.68 $\pm$ 11.71 & $\triangleleft$ & 99.38 $\pm$ 14.47 & \bftab 104.0 $\pm$ 10.61 & $\triangleleft$ & 115.2 $\pm$ 23.64 & \bftab 101.1 $\pm$ 4.747 & $\triangleleft$ & 106.5 $\pm$ 2.921 \\ 
FriedmanArtificialDomain & 2.408 $\pm$ 0.004 &  & \bftab 2.402 $\pm$ 0.005 & \bftab 2.655 $\pm$ 0.003 & $\triangleleft$ & 2.691 $\pm$ 0.003 & \bftab 2.142 $\pm$ 0.001 & $\triangleleft$ & 2.364 $\pm$ 0.001 & 4.987 $\pm$ 0.002 &  & 4.987 $\pm$ 0.002 \\ 
california & \bftab 67046 $\pm$ 7482 &  & 68258 $\pm$ 3628 & \bftab 69902 $\pm$ 1688 & $\triangleleft$ & 71389 $\pm$ 2392 & \bftab 76531 $\pm$ 50443 & $\triangleleft$ & 82323 $\pm$ 66260 & \bftab 115 $\pm$ 2181 & $\triangleleft$ & 117 $\pm$ 1451 \\ 
bike & \bftab 4.379 $\pm$ 0.791 &  & 4.624 $\pm$ 2.850 & \bftab 6.804 $\pm$ 5.023 & $\triangleleft$ & 8.725 $\pm$ 0.687 & \bftab 62.82 $\pm$ 21.52 & $\triangleleft$ & 76.37 $\pm$ 28.42 & \bftab 182.9 $\pm$ 12.77 & $\triangleleft$ & 189.4 $\pm$ 8.528 \\ 
3d-spatial-network & \bftab 14.24 $\pm$ 0.333 & $\triangleleft$ & 14.75 $\pm$ 0.280 & \bftab 18.28 $\pm$ 0.031 & $\triangleleft$ & 18.69 $\pm$ 0.025 & \bftab 7.670 $\pm$ 0.101 & $\triangleleft$ & 8.382 $\pm$ 0.264 & \bftab 18.52 $\pm$ 0.022 & $\triangleleft$ & 18.92 $\pm$ 0.014 \\ 
Range-Queries-Aggregates & 116.9 $\pm$ 17.03 &  & \bftab 114.9 $\pm$ 57.91 & \bftab 132.7 $\pm$ 6.010 & $\triangleleft$ & 132.9 $\pm$ 5.929 & \bftab 61.28 $\pm$ 13.38 &  & 62.60 $\pm$ 8.728 & \bftab 268.6 $\pm$ 1.358 & $\triangleleft$ & 268.8 $\pm$ 1.265 \\ 
pp-gas-emission & \bftab 6.558 $\pm$ 0.082 & $\triangleleft$ & 6.881 $\pm$ 0.172 & \bftab 8.049 $\pm$ 0.022 & $\triangleleft$ & 8.320 $\pm$ 0.019 & \bftab 7.446 $\pm$ 0.013 & $\triangleleft$ & 8.768 $\pm$ 0.021 & \bftab 11.65 $\pm$ 0.022 & $\triangleleft$ & 11.76 $\pm$ 0.019 \\ 
GPU-Kernel-Performance & 198.8 $\pm$ 123.1 &  & \bftab 192.3 $\pm$ 250.1 & \bftab 283.0 $\pm$ 63.45 & $\triangleleft$ & 285.0 $\pm$ 55.05 & \bftab 38.14 $\pm$ 12.22 &  & 41.32 $\pm$ 11.77 & \bftab 369.6 $\pm$ 10.89 & $\triangleleft$ & 375.2 $\pm$ 9.477 \\ 
polution & \bftab 74.11 $\pm$ 5.493 &  & 75.78 $\pm$ 7.066 & \bftab 79.94 $\pm$ 1.227 & $\triangleleft$ & 82.31 $\pm$ 1.338 & \bftab 67.51 $\pm$ 5.513 & $\triangleleft$ & 71.68 $\pm$ 4.106 & \bftab 92.46 $\pm$ 2.127 & $\triangleleft$ & 95.90 $\pm$ 1.403  


==> Tables/phi_Over.tex <==
puma32H & 0.032 $\pm$ 0.000 &  & \bftab 0.029 $\pm$ 0.000 & 0.050 $\pm$ 0.000 & $\triangleright$ & \bftab 0.045 $\pm$ 0.000 & 0.031 $\pm$ 0.000 & $\triangleright$ & \bftab 0.012 $\pm$ 0.000 & 0.070 $\pm$ 0.000 &  & 0.070 $\pm$ 0.000 \\ 
cpusum & 10.73 $\pm$ 0.443 &  & \bftab 8.959 $\pm$ 7.352 & \bftab 8.693 $\pm$ 0.830 & $\triangleleft$ & 10.15 $\pm$ 0.318 & \bftab 11.02 $\pm$ 0.744 &  & 11.40 $\pm$ 1.108 & 22.83 $\pm$ 1.568 & $\triangleright$ & \bftab 17.53 $\pm$ 2.044 \\ 
mv & \bftab 0.799 $\pm$ 0.034 &  & 0.835 $\pm$ 0.038 & 4.385 $\pm$ 0.002 & $\triangleright$ & \bftab 3.236 $\pm$ 0.001 & 1.278 $\pm$ 0.196 & $\triangleright$ & \bftab 0.748 $\pm$ 0.035 & 19.45 $\pm$ 0.002 & $\triangleright$ & \bftab 18.01 $\pm$ 0.002 \\ 
elevator & 0.144 $\pm$ 0.024 &  & \bftab 0.062 $\pm$ 0.004 & \bftab 0.073 $\pm$ 0.005 &  & 0.127 $\pm$ 0.015 & \bftab 0.016 $\pm$ 0.000 &  & 0.064 $\pm$ 0.024 & 0.020 $\pm$ 0.000 &  & 0.020 $\pm$ 0.000 \\ 
energydata-complete & 212.3 $\pm$ 5.919 & $\triangleright$ & \bftab 190.8 $\pm$ 4.632 & 202.9 $\pm$ 36.07 & $\triangleright$ & \bftab 184.4 $\pm$ 9.394 & 213.3 $\pm$ 17.65 & $\triangleright$ & \bftab 193.0 $\pm$ 11.07 & 223.1 $\pm$ 23.69 & $\triangleright$ & \bftab 201.2 $\pm$ 13.31 \\ 
FriedmanArtificialDomain & 3.385 $\pm$ 0.003 & $\triangleright$ & \bftab 3.076 $\pm$ 0.003 & 3.893 $\pm$ 0.000 & $\triangleright$ & \bftab 3.441 $\pm$ 0.000 & 2.890 $\pm$ 0.030 & $\triangleright$ & \bftab 2.217 $\pm$ 0.006 & 11.50 $\pm$ 0.001 &  & 11.50 $\pm$ 0.001 \\ 
california & 114 $\pm$ 1381 & $\triangleright$ & \bftab 102 $\pm$ 4526 & 120 $\pm$ 1120 & $\triangleright$ & \bftab 110 $\pm$ 660 & 110 $\pm$ 9471 & $\triangleright$ & \bftab 100 $\pm$ 9789 & 204 $\pm$ 989 & $\triangleright$ & \bftab 192 $\pm$ 959 \\ 
bike & 7.829 $\pm$ 6.136 &  & \bftab 7.456 $\pm$ 5.835 & 9.847 $\pm$ 2.514 &  & \bftab 9.665 $\pm$ 3.445 & 74.27 $\pm$ 31.46 &  & \bftab 70.16 $\pm$ 40.85 & 309.6 $\pm$ 1.051 & $\triangleright$ & \bftab 284.2 $\pm$ 1.385 \\ 
3d-spatial-network & 31.90 $\pm$ 0.814 & $\triangleright$ & \bftab 25.79 $\pm$ 0.146 & 43.14 $\pm$ 0.003 & $\triangleright$ & \bftab 40.04 $\pm$ 0.003 & 15.39 $\pm$ 1.707 & $\triangleright$ & \bftab 11.16 $\pm$ 0.291 & 44.90 $\pm$ 0.003 & $\triangleright$ & \bftab 42.43 $\pm$ 0.003 \\ 
Range-Queries-Aggregates & 200.0 $\pm$ 32.91 & $\triangleright$ & \bftab 186.5 $\pm$ 64.89 & 223.9 $\pm$ 0.581 & $\triangleright$ & \bftab 217.7 $\pm$ 0.571 & 101.7 $\pm$ 8.057 & $\triangleright$ & \bftab 92.29 $\pm$ 11.87 & \bftab 389.7 $\pm$ 0.297 & $\triangleleft$ & 391.0 $\pm$ 0.305 \\ 
pp-gas-emission & 14.65 $\pm$ 0.179 & $\triangleright$ & \bftab 12.96 $\pm$ 0.014 & 19.66 $\pm$ 0.033 & $\triangleright$ & \bftab 17.19 $\pm$ 0.054 & 16.08 $\pm$ 0.106 & $\triangleright$ & \bftab 13.76 $\pm$ 0.049 & 31.54 $\pm$ 0.049 & $\triangleright$ & \bftab 30.70 $\pm$ 0.047 \\ 
GPU-Kernel-Performance & 380.2 $\pm$ 236.0 & $\triangleright$ & \bftab 340.7 $\pm$ 65.37 & 551.0 $\pm$ 7.027 & $\triangleright$ & \bftab 422.3 $\pm$ 2.259 & 72.14 $\pm$ 21.20 &  & \bftab 61.48 $\pm$ 443.8 & 806.7 $\pm$ 6.551 & $\triangleright$ & \bftab 727.5 $\pm$ 8.634 \\ 
polution & 157.9 $\pm$ 15.78 & $\triangleright$ & \bftab 132.5 $\pm$ 4.074 & 175.2 $\pm$ 1.511 & $\triangleright$ & \bftab 150.0 $\pm$ 1.254 & 136.4 $\pm$ 7.201 & $\triangleright$ & \bftab 116.6 $\pm$ 24.60 & 211.5 $\pm$ 0.359 & $\triangleright$ & \bftab 192.6 $\pm$ 0.381


==> Tables/phi_Over_OLD.tex <==
puma32H & 0.033 $\pm$ 0.000 &  & \bftab 0.029 $\pm$ 0.000 & 0.050 $\pm$ 0.000 & $\triangleright$ & \bftab 0.044 $\pm$ 0.000 & 0.028 $\pm$ 0.000 & $\triangleright$ & \bftab 0.022 $\pm$ 0.000 & 0.070 $\pm$ 0.000 &  & 0.070 $\pm$ 0.000 \\ 
cpusum & 10.35 $\pm$ 2.908 & $\triangleright$ & \bftab 8.295 $\pm$ 4.873 & \bftab 9.323 $\pm$ 6.187 &  & 9.704 $\pm$ 3.513 & 13.45 $\pm$ 4.268 & $\triangleright$ & \bftab 10.40 $\pm$ 2.593 & 21.91 $\pm$ 1.992 & $\triangleright$ & \bftab 16.11 $\pm$ 2.329 \\ 
mv & 0.868 $\pm$ 0.143 &  & \bftab 0.628 $\pm$ 0.067 & 4.440 $\pm$ 0.067 & $\triangleright$ & \bftab 2.613 $\pm$ 0.044 & 1.050 $\pm$ 0.120 & $\triangleright$ & \bftab 0.562 $\pm$ 0.037 & 19.31 $\pm$ 0.064 & $\triangleright$ & \bftab 16.48 $\pm$ 0.063 \\ 
elevator & 0.160 $\pm$ 0.090 &  & \bftab 0.041 $\pm$ 0.004 & \bftab 0.019 $\pm$ 0.000 &  & 0.129 $\pm$ 0.060 & \bftab 0.064 $\pm$ 0.026 &  & 4.266 $\pm$ 104.4 & 0.020 $\pm$ 0.000 &  & 0.020 $\pm$ 0.000 \\ 
energydata-complete & 205.2 $\pm$ 38.86 & $\triangleright$ & \bftab 180.8 $\pm$ 42.73 & 199.0 $\pm$ 51.27 & $\triangleright$ & \bftab 178.3 $\pm$ 39.63 & 211.0 $\pm$ 73.97 & $\triangleright$ & \bftab 187.1 $\pm$ 68.76 & 222.3 $\pm$ 19.79 & $\triangleright$ & \bftab 192.8 $\pm$ 19.44 \\ 
FriedmanArtificialDomain & 3.364 $\pm$ 0.041 & $\triangleright$ & \bftab 2.829 $\pm$ 0.024 & 3.945 $\pm$ 0.090 & $\triangleright$ & \bftab 3.323 $\pm$ 0.081 & 2.745 $\pm$ 0.061 & $\triangleright$ & \bftab 2.041 $\pm$ 0.036 & \bftab 11.44 $\pm$ 0.034 &  & 11.44 $\pm$ 0.033 \\ 
california & 112 $\pm$ 30294 & $\triangleright$ & \bftab 101 $\pm$ 26902 & 121 $\pm$ 28373 & $\triangleright$ & \bftab 110 $\pm$ 30008 & 106 $\pm$ 53091 & $\triangleright$ & \bftab 98169 $\pm$ 50077 & 204 $\pm$ 8301 & $\triangleright$ & \bftab 186 $\pm$ 8508 \\ 
bike & \bftab 6.209 $\pm$ 3.896 &  & 9.221 $\pm$ 49.68 & 7.635 $\pm$ 8.615 & $\triangleright$ & \bftab 7.043 $\pm$ 8.010 & \bftab 69.50 $\pm$ 49.00 &  & 69.94 $\pm$ 46.47 & 310.9 $\pm$ 63.07 & $\triangleright$ & \bftab 258.3 $\pm$ 58.95 \\ 
3d-spatial-network & 30.63 $\pm$ 2.369 & $\triangleright$ & \bftab 25.98 $\pm$ 1.458 & 43.19 $\pm$ 0.186 & $\triangleright$ & \bftab 37.55 $\pm$ 0.219 & 13.28 $\pm$ 0.379 & $\triangleright$ & \bftab 9.989 $\pm$ 0.517 & 44.55 $\pm$ 0.112 & $\triangleright$ & \bftab 39.65 $\pm$ 0.112 \\ 
Range-Queries-Aggregates & 198.7 $\pm$ 36.29 & $\triangleright$ & \bftab 183.9 $\pm$ 171.5 & 222.4 $\pm$ 17.05 & $\triangleright$ & \bftab 218.3 $\pm$ 16.70 & 96.33 $\pm$ 54.07 & $\triangleright$ & \bftab 83.46 $\pm$ 43.76 & \bftab 389.6 $\pm$ 10.17 & $\triangleleft$ & 392.4 $\pm$ 9.607 \\ 
pp-gas-emission & 14.42 $\pm$ 0.617 & $\triangleright$ & \bftab 13.02 $\pm$ 0.666 & 19.91 $\pm$ 0.480 & $\triangleright$ & \bftab 17.13 $\pm$ 0.426 & 14.99 $\pm$ 0.960 & $\triangleright$ & \bftab 12.73 $\pm$ 0.782 & 31.72 $\pm$ 0.634 & $\triangleright$ & \bftab 30.28 $\pm$ 0.675 \\ 
GPU-Kernel-Performance & 384.4 $\pm$ 543.9 & $\triangleright$ & \bftab 360.1 $\pm$ 396.2 & 546.5 $\pm$ 397.9 & $\triangleright$ & \bftab 494.2 $\pm$ 399.2 & 60.55 $\pm$ 48.53 & $\triangleright$ & \bftab 45.49 $\pm$ 160.7 & 809.7 $\pm$ 73.35 & $\triangleright$ & \bftab 746.8 $\pm$ 78.06 \\ 
polution & 156.4 $\pm$ 47.61 & $\triangleright$ & \bftab 130.2 $\pm$ 29.60 & 177.2 $\pm$ 16.77 & $\triangleright$ & \bftab 148.6 $\pm$ 21.68 & 136.1 $\pm$ 58.24 & $\triangleright$ & \bftab 116.3 $\pm$ 51.41 & 211.4 $\pm$ 9.258 & $\triangleright$ & \bftab 182.3 $\pm$ 11.48  


==> Tables/phi_Un_OS.tex <==
puma32H & 0.03 $\pm$ 0.00 &  & \bftab 0.03 $\pm$ 0.00 & 0.04 $\pm$ 0.00 &  & \bftab 0.04 $\pm$ 0.00 & 0.04 $\pm$ 0.00 & $\triangleright$ & \bftab 0.02 $\pm$ 0.00 & 0.07 $\pm$ 0.00 &  & 0.07 $\pm$ 0.00 \\ 
cpusum & 9.96 $\pm$ 1.91 &  & \bftab 9.62 $\pm$ 6.98 & 10.25 $\pm$ 1.08 &  & \bftab 10.05 $\pm$ 0.75 & 20.78 $\pm$ 0.77 & $\triangleright$ & \bftab 11.61 $\pm$ 0.83 & 18.42 $\pm$ 0.86 & $\triangleright$ & \bftab 17.63 $\pm$ 0.97 \\ 
mv & \bftab 0.62 $\pm$ 0.06 &  & 0.68 $\pm$ 0.01 & 2.95 $\pm$ 0.01 & $\triangleright$ & \bftab 2.59 $\pm$ 0.00 & 2.07 $\pm$ 0.12 & $\triangleright$ & \bftab 0.71 $\pm$ 0.03 & 17.23 $\pm$ 0.01 & $\triangleright$ & \bftab 16.61 $\pm$ 0.01 \\ 
elevator & 0.12 $\pm$ 0.01 & $\triangleright$ & \bftab 0.06 $\pm$ 0.00 & \bftab 0.06 $\pm$ 0.00 &  & 0.11 $\pm$ 0.01 & \bftab 0.02 $\pm$ 0.00 & $\triangleleft$ & 7e+06 $\pm$ 4e+14 & 0.02 $\pm$ 0.00 &  & 0.02 $\pm$ 0.00 \\ 
energydata-complete & 194.02 $\pm$ 9.79 & $\triangleright$ & \bftab 187.76 $\pm$ 4.77 & 186.83 $\pm$ 3.19 & $\triangleright$ & \bftab 183.79 $\pm$ 3.31 & 208.55 $\pm$ 9.45 & $\triangleright$ & \bftab 194.74 $\pm$ 11.41 & 202.09 $\pm$ 6.38 & $\triangleright$ & \bftab 195.97 $\pm$ 6.12 \\ 
FriedmanArtificialDomain & 3.16 $\pm$ 0.01 & $\triangleright$ & \bftab 2.97 $\pm$ 0.01 & 3.33 $\pm$ 0.00 & $\triangleright$ & \bftab 3.27 $\pm$ 0.00 & 3.04 $\pm$ 0.01 & $\triangleright$ & \bftab 2.32 $\pm$ 0.02 & \bftab 11.49 $\pm$ 0.00 &  & 11.49 $\pm$ 0.00 \\ 
california & 1e+05 $\pm$ 4e+06 & $\triangleright$ & \bftab 1e+05 $\pm$ 3e+06 & 1e+05 $\pm$ 3e+06 & $\triangleright$ & \bftab 1e+05 $\pm$ 2e+06 & 1e+05 $\pm$ 7e+06 & $\triangleright$ & \bftab 1e+05 $\pm$ 2e+06 & 2e+05 $\pm$ 2e+06 & $\triangleright$ & \bftab 2e+05 $\pm$ 8e+05 \\ 
bike & \bftab 7.46 $\pm$ 5.80 &  & 11.15 $\pm$ 15.71 & 12.21 $\pm$ 1.44 & $\triangleright$ & \bftab 8.38 $\pm$ 17.23 & 94.35 $\pm$ 62.98 & $\triangleright$ & \bftab 78.53 $\pm$ 34.68 & 266.29 $\pm$ 5.25 & $\triangleright$ & \bftab 256.61 $\pm$ 7.91 \\ 
3d-spatial-network & 29.58 $\pm$ 1.20 & $\triangleright$ & \bftab 26.44 $\pm$ 0.29 & 39.14 $\pm$ 0.01 & $\triangleright$ & \bftab 37.48 $\pm$ 0.01 & 15.28 $\pm$ 0.31 & $\triangleright$ & \bftab 11.48 $\pm$ 0.18 & 41.43 $\pm$ 0.01 & $\triangleright$ & \bftab 40.00 $\pm$ 0.01 \\ 
Range-Queries-Aggregates & 197.70 $\pm$ 74.11 & $\triangleright$ & \bftab 190.19 $\pm$ 80.00 & 221.64 $\pm$ 1.10 & $\triangleright$ & \bftab 220.00 $\pm$ 1.11 & 108.15 $\pm$ 14.20 & $\triangleright$ & \bftab 94.89 $\pm$ 12.98 & 393.06 $\pm$ 0.22 & $\triangleright$ & \bftab 392.78 $\pm$ 0.17 \\ 
pp-gas-emission & 13.98 $\pm$ 0.05 & $\triangleright$ & \bftab 13.21 $\pm$ 0.06 & 17.99 $\pm$ 0.03 & $\triangleright$ & \bftab 17.14 $\pm$ 0.02 & 16.66 $\pm$ 0.13 & $\triangleright$ & \bftab 14.32 $\pm$ 0.08 & 30.51 $\pm$ 0.01 & $\triangleright$ & \bftab 30.18 $\pm$ 0.02 \\ 
GPU-Kernel-Performance & 364.31 $\pm$ 73.10 &  & \bftab 356.56 $\pm$ 43.72 & 517.58 $\pm$ 2.31 & $\triangleright$ & \bftab 498.92 $\pm$ 3.33 & 97.32 $\pm$ 70.31 & $\triangleright$ & \bftab 56.15 $\pm$ 268.71 & 764.18 $\pm$ 9.11 & $\triangleright$ & \bftab 745.16 $\pm$ 9.93 \\ 
polution & 143.92 $\pm$ 2.69 & $\triangleright$ & \bftab 133.23 $\pm$ 2.38 & 152.16 $\pm$ 16.89 & $\triangleright$ & \bftab 144.64 $\pm$ 26.09 & 133.68 $\pm$ 114.34 & $\triangleright$ & \bftab 125.78 $\pm$ 120.82 & 177.06 $\pm$ 583.32 & $\triangleright$ & \bftab 170.56 $\pm$ 616.93


==> Tables/phi_Under.tex <==
puma32H & 0.032 $\pm$ 0.000 &  & \bftab 0.028 $\pm$ 0.000 & 0.050 $\pm$ 0.000 & $\triangleright$ & \bftab 0.040 $\pm$ 0.000 & \bftab 0.031 $\pm$ 0.000 & $\triangleleft$ & 0.046 $\pm$ 0.000 & 0.070 $\pm$ 0.000 &  & 0.070 $\pm$ 0.000 \\ 
cpusum & \bftab 10.73 $\pm$ 0.443 & $\triangleleft$ & 16.29 $\pm$ 5.629 & \bftab 8.693 $\pm$ 0.830 & $\triangleleft$ & 25.25 $\pm$ 75.01 & \bftab 11.02 $\pm$ 0.744 & $\triangleleft$ & 55.90 $\pm$ 43.12 & 22.83 $\pm$ 1.568 & $\triangleright$ & \bftab 14.49 $\pm$ 0.495 \\ 
mv & 0.799 $\pm$ 0.034 & $\triangleright$ & \bftab 0.573 $\pm$ 0.033 & 4.385 $\pm$ 0.002 & $\triangleright$ & \bftab 1.397 $\pm$ 0.002 & \bftab 1.278 $\pm$ 0.196 & $\triangleleft$ & 2.941 $\pm$ 0.031 & 19.45 $\pm$ 0.002 & $\triangleright$ & \bftab 12.60 $\pm$ 0.003 \\ 
elevator & 0.144 $\pm$ 0.024 &  & \bftab 0.061 $\pm$ 0.004 & 0.073 $\pm$ 0.005 &  & \bftab 0.046 $\pm$ 0.001 & 0.016 $\pm$ 0.000 &  & \bftab 0.010 $\pm$ 0.000 & 0.020 $\pm$ 0.000 & $\triangleright$ & \bftab 0.010 $\pm$ 0.000 \\ 
energydata-complete & 212.3 $\pm$ 5.919 & $\triangleright$ & \bftab 173.7 $\pm$ 4.999 & 202.9 $\pm$ 36.07 & $\triangleright$ & \bftab 172.0 $\pm$ 10.29 & 213.3 $\pm$ 17.65 &  & \bftab 212.5 $\pm$ 194.6 & 223.1 $\pm$ 23.69 & $\triangleright$ & \bftab 160.5 $\pm$ 487.2 \\ 
FriedmanArtificialDomain & 3.385 $\pm$ 0.003 & $\triangleright$ & \bftab 2.771 $\pm$ 0.006 & 3.893 $\pm$ 0.000 & $\triangleright$ & \bftab 2.801 $\pm$ 0.001 & 2.890 $\pm$ 0.030 &  & \bftab 2.791 $\pm$ 0.030 & 11.50 $\pm$ 0.001 &  & \bftab 11.50 $\pm$ 0.001 \\ 
california & 114 $\pm$ 1381 & $\triangleright$ & \bftab 91877 $\pm$ 5799 & 120 $\pm$ 1120 & $\triangleright$ & \bftab 98194 $\pm$ 8950 & 110 $\pm$ 9471 & $\triangleright$ & \bftab 101 $\pm$ 11846 & 204 $\pm$ 989 & $\triangleright$ & \bftab 159 $\pm$ 2211 \\ 
bike & \bftab 7.829 $\pm$ 6.136 &  & 9.007 $\pm$ 6.718 & \bftab 9.847 $\pm$ 2.514 & $\triangleleft$ & 18.48 $\pm$ 6.987 & \bftab 74.27 $\pm$ 31.46 & $\triangleleft$ & 151.4 $\pm$ 133.5 & 309.6 $\pm$ 1.051 & $\triangleright$ & \bftab 183.0 $\pm$ 2.236 \\ 
3d-spatial-network & 31.90 $\pm$ 0.814 & $\triangleright$ & \bftab 21.44 $\pm$ 0.891 & 43.14 $\pm$ 0.003 & $\triangleright$ & \bftab 30.07 $\pm$ 0.004 & 15.39 $\pm$ 1.707 & $\triangleright$ & \bftab 13.01 $\pm$ 0.255 & 44.90 $\pm$ 0.003 & $\triangleright$ & \bftab 32.85 $\pm$ 0.010 \\ 
Range-Queries-Aggregates & 200.0 $\pm$ 32.91 &  & \bftab 194.7 $\pm$ 59.39 & 223.9 $\pm$ 0.581 & $\triangleright$ & \bftab 212.2 $\pm$ 0.615 & \bftab 101.7 $\pm$ 8.057 & $\triangleleft$ & 116.7 $\pm$ 31.72 & \bftab 389.7 $\pm$ 0.297 & $\triangleleft$ & 392.4 $\pm$ 0.390 \\ 
pp-gas-emission & 14.65 $\pm$ 0.179 & $\triangleright$ & \bftab 13.18 $\pm$ 0.059 & 19.66 $\pm$ 0.033 & $\triangleright$ & \bftab 15.98 $\pm$ 0.084 & \bftab 16.08 $\pm$ 0.106 & $\triangleleft$ & 16.53 $\pm$ 0.211 & 31.54 $\pm$ 0.049 & $\triangleright$ & \bftab 29.36 $\pm$ 0.059 \\ 
GPU-Kernel-Performance & 380.2 $\pm$ 236.0 & $\triangleright$ & \bftab 317.5 $\pm$ 178.3 & 551.0 $\pm$ 7.027 & $\triangleright$ & \bftab 377.4 $\pm$ 3.770 & \bftab 72.14 $\pm$ 21.20 & $\triangleleft$ & 214.6 $\pm$ 156.7 & 806.7 $\pm$ 6.551 & $\triangleright$ & \bftab 558.6 $\pm$ 4.713 \\ 
polution & 157.9 $\pm$ 15.78 & $\triangleright$ & \bftab 105.6 $\pm$ 7.552 & 175.2 $\pm$ 1.511 & $\triangleright$ & \bftab 105.8 $\pm$ 2.012 & 136.4 $\pm$ 7.201 & $\triangleright$ & \bftab 103.3 $\pm$ 7.349 & 211.5 $\pm$ 0.359 & $\triangleright$ & \bftab 132.2 $\pm$ 0.680


==> Tables/phi_Under_OLD.tex <==
puma32H & \bftab 0.033 $\pm$ 0.000 &  & 0.034 $\pm$ 0.000 & 0.050 $\pm$ 0.000 & $\triangleright$ & \bftab 0.043 $\pm$ 0.000 & \bftab 0.028 $\pm$ 0.000 & $\triangleleft$ & 0.034 $\pm$ 0.000 & 0.070 $\pm$ 0.000 &  & 0.070 $\pm$ 0.000 \\ 
cpusum & 10.35 $\pm$ 2.908 & $\triangleright$ & \bftab 8.934 $\pm$ 5.048 & \bftab 9.323 $\pm$ 6.187 & $\triangleleft$ & 10.58 $\pm$ 4.889 & \bftab 13.45 $\pm$ 4.268 & $\triangleleft$ & 20.69 $\pm$ 7.831 & 21.91 $\pm$ 1.992 & $\triangleright$ & \bftab 16.98 $\pm$ 2.250 \\ 
mv & 0.868 $\pm$ 0.143 & $\triangleright$ & \bftab 0.401 $\pm$ 0.042 & 4.440 $\pm$ 0.067 & $\triangleright$ & \bftab 2.941 $\pm$ 0.053 & 1.050 $\pm$ 0.120 &  & \bftab 0.943 $\pm$ 0.076 & 19.31 $\pm$ 0.064 & $\triangleright$ & \bftab 17.09 $\pm$ 0.070 \\ 
elevator & \bftab 0.160 $\pm$ 0.090 &  & 0.213 $\pm$ 0.098 & 0.019 $\pm$ 0.000 &  & \bftab 0.018 $\pm$ 0.000 & 0.064 $\pm$ 0.026 &  & \bftab 0.014 $\pm$ 0.000 & 0.020 $\pm$ 0.000 &  & 0.020 $\pm$ 0.000 \\ 
energydata-complete & 205.2 $\pm$ 38.86 & $\triangleright$ & \bftab 187.6 $\pm$ 43.54 & 199.0 $\pm$ 51.27 & $\triangleright$ & \bftab 182.2 $\pm$ 46.83 & 211.0 $\pm$ 73.97 & $\triangleright$ & \bftab 198.8 $\pm$ 116.8 & 222.3 $\pm$ 19.79 & $\triangleright$ & \bftab 199.3 $\pm$ 20.04 \\ 
FriedmanArtificialDomain & 3.364 $\pm$ 0.041 & $\triangleright$ & \bftab 2.896 $\pm$ 0.025 & 3.945 $\pm$ 0.090 & $\triangleright$ & \bftab 3.380 $\pm$ 0.087 & 2.745 $\pm$ 0.061 &  & \bftab 2.702 $\pm$ 0.045 & 11.44 $\pm$ 0.034 &  & 11.44 $\pm$ 0.034 \\ 
california & 112 $\pm$ 30294 & $\triangleright$ & \bftab 104 $\pm$ 40599 & 121 $\pm$ 28373 & $\triangleright$ & \bftab 111 $\pm$ 39224 & 106 $\pm$ 53091 & $\triangleright$ & \bftab 102 $\pm$ 50926 & 204 $\pm$ 8301 & $\triangleright$ & \bftab 186 $\pm$ 8903 \\ 
bike & 6.209 $\pm$ 3.896 &  & \bftab 6.190 $\pm$ 9.474 & \bftab 7.635 $\pm$ 8.615 & $\triangleleft$ & 9.733 $\pm$ 4.095 & \bftab 69.50 $\pm$ 49.00 & $\triangleleft$ & 81.19 $\pm$ 74.17 & 310.9 $\pm$ 63.07 & $\triangleright$ & \bftab 269.0 $\pm$ 61.93 \\ 
3d-spatial-network & 30.63 $\pm$ 2.369 & $\triangleright$ & \bftab 27.84 $\pm$ 2.469 & 43.19 $\pm$ 0.186 & $\triangleright$ & \bftab 39.18 $\pm$ 0.206 & \bftab 13.28 $\pm$ 0.379 &  & 13.50 $\pm$ 1.350 & 44.55 $\pm$ 0.112 & $\triangleright$ & \bftab 41.09 $\pm$ 0.112 \\ 
Range-Queries-Aggregates & 198.7 $\pm$ 36.29 &  & \bftab 196.5 $\pm$ 150.0 & 222.4 $\pm$ 17.05 & $\triangleright$ & \bftab 219.9 $\pm$ 16.68 & \bftab 96.33 $\pm$ 54.07 &  & 97.03 $\pm$ 41.97 & \bftab 389.6 $\pm$ 10.17 & $\triangleleft$ & 392.5 $\pm$ 9.734 \\ 
pp-gas-emission & 14.42 $\pm$ 0.617 &  & \bftab 13.72 $\pm$ 0.482 & 19.91 $\pm$ 0.480 & $\triangleright$ & \bftab 17.96 $\pm$ 0.563 & \bftab 14.99 $\pm$ 0.960 &  & 15.23 $\pm$ 0.812 & 31.72 $\pm$ 0.634 & $\triangleright$ & \bftab 30.58 $\pm$ 0.692 \\ 
GPU-Kernel-Performance & 384.4 $\pm$ 543.9 &  & \bftab 357.6 $\pm$ 1444 & 546.5 $\pm$ 397.9 & $\triangleright$ & \bftab 513.1 $\pm$ 374.2 & 60.55 $\pm$ 48.53 &  & \bftab 59.95 $\pm$ 7.913 & 809.7 $\pm$ 73.35 & $\triangleright$ & \bftab 765.6 $\pm$ 76.27 \\ 
polution & 156.4 $\pm$ 47.61 & $\triangleright$ & \bftab 138.7 $\pm$ 75.37 & 177.2 $\pm$ 16.77 & $\triangleright$ & \bftab 156.1 $\pm$ 18.94 & 136.1 $\pm$ 58.24 & $\triangleright$ & \bftab 126.2 $\pm$ 55.15 & 211.4 $\pm$ 9.258 & $\triangleright$ & \bftab 188.5 $\pm$ 10.17 


==> Tables/right_OS_phi_8_.tex <==
puma32H & 0.04 $\pm$ 0.0 & $\triangleright$ & \bftab 0.03 $\pm$ 0.0 & 0.03 $\pm$ 0.01 & $\triangleright$ & \bftab 0.02 $\pm$ 0.0 & 0.04 $\pm$ 0.0 & $\triangleright$ & \bftab 0.02 $\pm$ 0.01 & 0.04 $\pm$ 0.0 & $\triangleright$ & \bftab 0.02 $\pm$ 0.0 \\
cpusum & 27.37 $\pm$ 1.22 & $\triangleright$ & \bftab 14.04 $\pm$ 0.4 & 22.61 $\pm$ 1.97 & $\triangleright$ & \bftab 13.37 $\pm$ 0.36 & 33.25 $\pm$ 4.23 & $\triangleright$ & \bftab 23.97 $\pm$ 3.5 & 34.99 $\pm$ 1.16 & $\triangleright$ & \bftab 25.88 $\pm$ 0.73 \\
elevator & 0.0 $\pm$ 0.0 & & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & & 0.0 $\pm$ 0.0 \\
bike & 6.2 $\pm$ 2.08 & $\triangleright$ & \bftab 1.93 $\pm$ 0.14 & 32.05 $\pm$ 5.37 & $\triangleright$ & \bftab 8.89 $\pm$ 1.53 & 88.24 $\pm$ 14.53 & $\triangleright$ & \bftab 18.8 $\pm$ 2.61 & 93.81 $\pm$ 4.01 & $\triangleright$ & \bftab 19.57 $\pm$ 0.83 \\
energy & 55.68 $\pm$ 1.68 & $\triangleright$ & \bftab 22.73 $\pm$ 0.39 & 53.84 $\pm$ 0.57 & $\triangleright$ & \bftab 22.29 $\pm$ 0.11 & 57.81 $\pm$ 1.6 & $\triangleright$ & \bftab 23.25 $\pm$ 0.36 & 58.49 $\pm$ 0.56 & $\triangleright$ & \bftab 23.33 $\pm$ 0.1 \\
calhousing & $46\times10^3$ $\pm$ 864.44 & $\triangleright$ & \bftab $31\times10^3$ $\pm$ 424.77 & $46\times10^3$ $\pm$ 855.59 & $\triangleright$ & \bftab $29\times10^3$ $\pm$ 879.89 & $77\times10^3$ $\pm$ $93\times10^2$ & $\triangleright$ & \bftab $35\times10^3$ $\pm$ $24\times10^2$ & $81\times10^3$ $\pm$ $23\times10^2$ & $\triangleright$ & \bftab $36\times10^3$ $\pm$ 625.17 \\
gasemission & 14.47 $\pm$ 0.6 & $\triangleright$ & \bftab 10.87 $\pm$ 0.18 & 14.08 $\pm$ 0.19 & $\triangleright$ & \bftab 10.57 $\pm$ 0.19 & 15.71 $\pm$ 0.9 & $\triangleright$ & \bftab 10.86 $\pm$ 0.29 & 16.03 $\pm$ 0.39 & $\triangleright$ & \bftab 10.94 $\pm$ 0.14 \\
mv & 5.18 $\pm$ 0.16 & $\triangleright$ & \bftab 0.04 $\pm$ 0.1 & 4.41 $\pm$ 1.28 & $\triangleright$ & \bftab 1.0 $\pm$ 1.16 & 11.96 $\pm$ 1.6 & $\triangleright$ & \bftab 6.81 $\pm$ 1.0 & 12.09 $\pm$ 0.48 & $\triangleright$ & \bftab 6.95 $\pm$ 0.28 \\
fried & \bftab 2.98 $\pm$ 0.21 & & 2.99 $\pm$ 0.16 & 2.88 $\pm$ 0.09 & $\triangleright$ & \bftab 2.71 $\pm$ 0.13 & 5.62 $\pm$ 0.78 & $\triangleright$ & \bftab 3.76 $\pm$ 0.37 & 5.91 $\pm$ 0.22 & $\triangleright$ & \bftab 3.88 $\pm$ 0.1 \\
polution & 53.97 $\pm$ 0.22 & $\triangleright$ & \bftab 15.86 $\pm$ 0.09 & 48.84 $\pm$ 1.68 & $\triangleright$ & \bftab 15.35 $\pm$ 0.13 & 56.13 $\pm$ 3.15 & $\triangleright$ & \bftab 16.14 $\pm$ 0.34 & 57.0 $\pm$ 1.11 & $\triangleright$ & \bftab 16.12 $\pm$ 0.17 \\
car price & $22\times10^3$ $\pm$ $64\times10^2$ & $\triangleright$ & \bftab $32\times10^2$ $\pm$ $10\times10^2$ & $60\times10^3$ $\pm$ $17\times10^3$ & $\triangleright$ & \bftab $67\times10^2$ $\pm$ $18\times10^2$ & $61\times10^3$ $\pm$ $36\times10^2$ & $\triangleright$ & \bftab $58\times10^2$ $\pm$ 308.45 & $53\times10^3$ $\pm$ $17\times10^2$ & $\triangleright$ & \bftab $50\times10^2$ $\pm$ 167.69 \\
query & 345.12 $\pm$ 1.98 & $\triangleright$ & \bftab 207.23 $\pm$ 1.39 & 285.34 $\pm$ 20.14 & $\triangleright$ & \bftab 170.98 $\pm$ 12.05 & 370.06 $\pm$ 34.16 & $\triangleright$ & \bftab 224.39 $\pm$ 21.27 & 393.31 $\pm$ 5.67 & $\triangleright$ & \bftab 234.93 $\pm$ 4.91 \\
GPU & 134.41 $\pm$ 0.41 & $\triangleright$ & \bftab 11.47 $\pm$ 0.02 & 108.82 $\pm$ 12.54 & $\triangleright$ & \bftab 9.55 $\pm$ 0.96 & 116.25 $\pm$ 10.56 & $\triangleright$ & \bftab 10.72 $\pm$ 1.1 & 118.66 $\pm$ 4.62 & $\triangleright$ & \bftab 11.36 $\pm$ 0.29 \\
3d & 19.87 $\pm$ 0.55 & $\triangleright$ & \bftab 8.24 $\pm$ 0.69 & 16.87 $\pm$ 1.56 & $\triangleright$ & \bftab 7.19 $\pm$ 0.41 & 16.3 $\pm$ 0.72 & $\triangleright$ & \bftab 6.96 $\pm$ 0.17 & 16.89 $\pm$ 0.2 & $\triangleright$ & \bftab 7.14 $\pm$ 0.05 \\


==> Tables/right_US_phi_8_.tex <==
puma32H & 0.04 $\pm$ 0.0 & $\triangleright$ & \bftab 0.02 $\pm$ 0.0 & 0.03 $\pm$ 0.01 & $\triangleright$ & \bftab 0.02 $\pm$ 0.0 & 0.04 $\pm$ 0.0 & $\triangleright$ & \bftab 0.02 $\pm$ 0.0 & 0.04 $\pm$ 0.0 & $\triangleright$ & \bftab 0.02 $\pm$ 0.0 \\
cpusum & 27.37 $\pm$ 1.22 & & \bftab 19.58 $\pm$ 8.93 & \bftab 22.61 $\pm$ 1.97 & $\triangleleft$ & 35.28 $\pm$ 1.73 & \bftab 33.25 $\pm$ 4.23 & & 35.1 $\pm$ 0.16 & 34.99 $\pm$ 1.16 & $\triangleright$ & \bftab 32.2 $\pm$ 1.07 \\
elevator & 0.0 $\pm$ 0.0 & & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & & 0.0 $\pm$ 0.0 & 0.0 $\pm$ 0.0 & & 0.0 $\pm$ 0.0 \\
bike & \bftab 6.2 $\pm$ 2.08 & $\triangleleft$ & 24.0 $\pm$ 3.58 & \bftab 32.05 $\pm$ 5.37 & $\triangleleft$ & 44.1 $\pm$ 5.53 & 88.24 $\pm$ 14.53 & $\triangleright$ & \bftab 44.25 $\pm$ 2.27 & 93.81 $\pm$ 4.01 & $\triangleright$ & \bftab 38.5 $\pm$ 1.36 \\
energy & 55.68 $\pm$ 1.68 & $\triangleright$ & \bftab 17.73 $\pm$ 0.06 & 53.84 $\pm$ 0.57 & $\triangleright$ & \bftab 17.77 $\pm$ 0.01 & 57.81 $\pm$ 1.6 & $\triangleright$ & \bftab 17.77 $\pm$ 0.01 & 58.49 $\pm$ 0.56 & $\triangleright$ & \bftab 17.79 $\pm$ 0.01 \\
calhousing & $46\times10^3$ $\pm$ 864.44 & $\triangleright$ & \bftab $24\times10^3$ $\pm$ 703.84 & $46\times10^3$ $\pm$ 855.59 & $\triangleright$ & \bftab $25\times10^3$ $\pm$ 152.89 & $77\times10^3$ $\pm$ $93\times10^2$ & $\triangleright$ & \bftab $28\times10^3$ $\pm$ $10\times10^2$ & $81\times10^3$ $\pm$ $23\times10^2$ & $\triangleright$ & \bftab $28\times10^3$ $\pm$ 363.34 \\
gasemission & 14.47 $\pm$ 0.6 & $\triangleright$ & \bftab 9.51 $\pm$ 0.18 & 14.08 $\pm$ 0.19 & $\triangleright$ & \bftab 9.65 $\pm$ 0.21 & 15.71 $\pm$ 0.9 & $\triangleright$ & \bftab 9.84 $\pm$ 0.07 & 16.03 $\pm$ 0.39 & $\triangleright$ & \bftab 9.78 $\pm$ 0.09 \\
mv & 5.18 $\pm$ 0.16 & $\triangleright$ & \bftab 0.07 $\pm$ 0.19 & 4.41 $\pm$ 1.28 & $\triangleright$ & \bftab 1.52 $\pm$ 0.7 & 11.96 $\pm$ 1.6 & $\triangleright$ & \bftab 5.23 $\pm$ 0.71 & 12.09 $\pm$ 0.48 & $\triangleright$ & \bftab 5.29 $\pm$ 0.21 \\
fried & 2.98 $\pm$ 0.21 & $\triangleright$ & \bftab 2.31 $\pm$ 0.15 & 2.88 $\pm$ 0.09 & $\triangleright$ & \bftab 2.32 $\pm$ 0.03 & 5.62 $\pm$ 0.78 & $\triangleright$ & \bftab 3.12 $\pm$ 0.26 & 5.91 $\pm$ 0.22 & $\triangleright$ & \bftab 3.22 $\pm$ 0.07 \\
polution & \bftab 53.97 $\pm$ 0.22 & & 65.93 $\pm$ 63.68 & \bftab 48.84 $\pm$ 1.68 & $\triangleleft$ & 71.33 $\pm$ 5.3 & \bftab 56.13 $\pm$ 3.15 & & 57.07 $\pm$ 3.33 & 57.0 $\pm$ 1.11 & $\triangleright$ & \bftab 48.43 $\pm$ 2.03 \\
car price & $22\times10^3$ $\pm$ $64\times10^2$ & $\triangleright$ & \bftab 999.9 $\pm$ 2.32 & $60\times10^3$ $\pm$ $17\times10^3$ & $\triangleright$ & \bftab $10\times10^2$ $\pm$ 0.52 & $61\times10^3$ $\pm$ $36\times10^2$ & $\triangleright$ & \bftab $10\times10^2$ $\pm$ 0.32 & $53\times10^3$ $\pm$ $17\times10^2$ & $\triangleright$ & \bftab $10\times10^2$ $\pm$ 0.21 \\
query & 345.12 $\pm$ 1.98 & $\triangleright$ & \bftab 166.71 $\pm$ 1.44 & 285.34 $\pm$ 20.14 & $\triangleright$ & \bftab 146.21 $\pm$ 6.89 & 370.06 $\pm$ 34.16 & $\triangleright$ & \bftab 186.07 $\pm$ 15.32 & 393.31 $\pm$ 5.67 & $\triangleright$ & \bftab 193.81 $\pm$ 3.57 \\
GPU & 134.41 $\pm$ 0.41 & $\triangleright$ & \bftab 21.91 $\pm$ 0.01 & 108.82 $\pm$ 12.54 & $\triangleright$ & \bftab 21.9 $\pm$ 0.01 & 116.25 $\pm$ 10.56 & $\triangleright$ & \bftab 21.91 $\pm$ 0.0 & 118.66 $\pm$ 4.62 & $\triangleright$ & \bftab 21.91 $\pm$ 0.0 \\
3d & 19.87 $\pm$ 0.55 & $\triangleright$ & \bftab 6.33 $\pm$ 0.67 & 16.87 $\pm$ 1.56 & $\triangleright$ & \bftab 5.92 $\pm$ 0.17 & 16.3 $\pm$ 0.72 & $\triangleright$ & \bftab 5.84 $\pm$ 0.07 & 16.89 $\pm$ 0.2 & $\triangleright$ & \bftab 5.86 $\pm$ 0.04 \\


==> Tables/sera_Over.tex <==
puma32H & 0.550 $\pm$ 0.001 &  & \bftab 0.527 $\pm$ 0.001 & 0.644 $\pm$ 0.000 & $\triangleright$ & \bftab 0.605 $\pm$ 0.000 & 0.472 $\pm$ 0.002 & $\triangleright$ & \bftab 0.412 $\pm$ 0.001 & 0.750 $\pm$ 0.000 &  & 0.750 $\pm$ 0.000 \\ 
cpusum & \bftab 0.460 $\pm$ 0.001 &  & 0.467 $\pm$ 0.003 & 0.317 $\pm$ 0.000 & $\triangleright$ & \bftab 0.301 $\pm$ 0.000 & \bftab 0.473 $\pm$ 0.000 & $\triangleleft$ & 0.501 $\pm$ 0.000 & 0.356 $\pm$ 0.000 & $\triangleright$ & \bftab 0.300 $\pm$ 0.000 \\ 
mv & 0.508 $\pm$ 0.001 &  & \bftab 0.490 $\pm$ 0.001 & 0.520 $\pm$ 0.000 & $\triangleright$ & \bftab 0.486 $\pm$ 0.000 & 0.760 $\pm$ 0.002 & $\triangleright$ & \bftab 0.726 $\pm$ 0.001 & 0.747 $\pm$ 0.000 & $\triangleright$ & \bftab 0.689 $\pm$ 0.000 \\ 
elevator & \bftab 0.887 $\pm$ 0.011 &  & 0.891 $\pm$ 0.012 & 0.945 $\pm$ 0.002 &  & \bftab 0.937 $\pm$ 0.005 & 0.815 $\pm$ 0.006 &  & \bftab 0.800 $\pm$ 0.006 & 0.921 $\pm$ 0.000 &  & 0.921 $\pm$ 0.000 \\ 
energydata-complete & 0.918 $\pm$ 0.000 & $\triangleright$ & \bftab 0.796 $\pm$ 0.000 & 0.906 $\pm$ 0.000 & $\triangleright$ & \bftab 0.792 $\pm$ 0.000 & 0.877 $\pm$ 0.000 & $\triangleright$ & \bftab 0.778 $\pm$ 0.000 & 0.903 $\pm$ 0.000 & $\triangleright$ & \bftab 0.774 $\pm$ 0.000 \\ 
FriedmanArtificialDomain & 0.359 $\pm$ 0.000 & $\triangleright$ & \bftab 0.326 $\pm$ 0.000 & 0.366 $\pm$ 0.000 & $\triangleright$ & \bftab 0.334 $\pm$ 0.000 & 0.340 $\pm$ 0.000 & $\triangleright$ & \bftab 0.300 $\pm$ 0.000 & 0.601 $\pm$ 0.000 &  & 0.601 $\pm$ 0.000 \\ 
california & \bftab 0.584 $\pm$ 0.000 & $\triangleleft$ & 0.596 $\pm$ 0.000 & \bftab 0.556 $\pm$ 0.000 & $\triangleleft$ & 0.558 $\pm$ 0.000 & \bftab 0.591 $\pm$ 0.000 & $\triangleleft$ & 0.605 $\pm$ 0.000 & \bftab 0.532 $\pm$ 0.000 & $\triangleleft$ & 0.534 $\pm$ 0.000 \\ 
bike & 0.891 $\pm$ 0.001 &  & \bftab 0.868 $\pm$ 0.001 & 0.770 $\pm$ 0.000 & $\triangleright$ & \bftab 0.763 $\pm$ 0.000 & 0.769 $\pm$ 0.000 &  & \bftab 0.766 $\pm$ 0.000 & 0.797 $\pm$ 0.000 & $\triangleright$ & \bftab 0.738 $\pm$ 0.000 \\ 
3d-spatial-network & 0.675 $\pm$ 0.000 & $\triangleright$ & \bftab 0.608 $\pm$ 0.000 & 0.679 $\pm$ 0.000 & $\triangleright$ & \bftab 0.604 $\pm$ 0.000 & 0.675 $\pm$ 0.000 & $\triangleright$ & \bftab 0.650 $\pm$ 0.000 & 0.696 $\pm$ 0.000 & $\triangleright$ & \bftab 0.627 $\pm$ 0.000 \\ 
Range-Queries-Aggregates & 0.921 $\pm$ 0.000 & $\triangleright$ & \bftab 0.911 $\pm$ 0.000 & 0.914 $\pm$ 0.000 & $\triangleright$ & \bftab 0.897 $\pm$ 0.000 & 0.898 $\pm$ 0.000 & $\triangleright$ & \bftab 0.886 $\pm$ 0.000 & 0.868 $\pm$ 0.000 & $\triangleright$ & \bftab 0.866 $\pm$ 0.000 \\ 
pp-gas-emission & 0.603 $\pm$ 0.000 & $\triangleright$ & \bftab 0.559 $\pm$ 0.000 & 0.626 $\pm$ 0.000 & $\triangleright$ & \bftab 0.556 $\pm$ 0.000 & 0.562 $\pm$ 0.000 & $\triangleright$ & \bftab 0.520 $\pm$ 0.000 & 0.735 $\pm$ 0.000 & $\triangleright$ & \bftab 0.708 $\pm$ 0.000 \\ 
GPU-Kernel-Performance & 0.858 $\pm$ 0.000 & $\triangleright$ & \bftab 0.846 $\pm$ 0.000 & 0.815 $\pm$ 0.000 & $\triangleright$ & \bftab 0.637 $\pm$ 0.000 & 0.744 $\pm$ 0.002 & $\triangleright$ & \bftab 0.590 $\pm$ 0.004 & 0.880 $\pm$ 0.000 & $\triangleright$ & \bftab 0.706 $\pm$ 0.000 \\ 
polution & 0.774 $\pm$ 0.000 & $\triangleright$ & \bftab 0.696 $\pm$ 0.000 & 0.770 $\pm$ 0.000 & $\triangleright$ & \bftab 0.669 $\pm$ 0.000 & 0.761 $\pm$ 0.000 & $\triangleright$ & \bftab 0.699 $\pm$ 0.000 & 0.772 $\pm$ 0.000 & $\triangleright$ & \bftab 0.666 $\pm$ 0.000


==> Tables/sera_Un_OS.tex <==
puma32H & 0.52 $\pm$ 0.00 &  & \bftab 0.50 $\pm$ 0.00 & \bftab 0.58 $\pm$ 0.00 &  & 0.58 $\pm$ 0.00 & 0.43 $\pm$ 0.00 &  & \bftab 0.43 $\pm$ 0.00 & 0.75 $\pm$ 0.00 &  & 0.75 $\pm$ 0.00 \\ 
cpusum & \bftab 0.33 $\pm$ 0.00 & $\triangleleft$ & 0.44 $\pm$ 0.01 & \bftab 0.31 $\pm$ 0.00 &  & 0.32 $\pm$ 0.00 & \bftab 0.43 $\pm$ 0.00 & $\triangleleft$ & 0.48 $\pm$ 0.00 & 0.31 $\pm$ 0.00 & $\triangleright$ & \bftab 0.30 $\pm$ 0.00 \\ 
mv & \bftab 0.46 $\pm$ 0.00 &  & 0.47 $\pm$ 0.00 & 0.47 $\pm$ 0.00 & $\triangleright$ & \bftab 0.46 $\pm$ 0.00 & 0.77 $\pm$ 0.00 & $\triangleright$ & \bftab 0.69 $\pm$ 0.00 & 0.66 $\pm$ 0.00 & $\triangleright$ & \bftab 0.63 $\pm$ 0.00 \\ 
elevator & 0.92 $\pm$ 0.01 &  & \bftab 0.89 $\pm$ 0.01 & \bftab 0.90 $\pm$ 0.01 &  & 0.93 $\pm$ 0.01 & 0.82 $\pm$ 0.01 &  & \bftab 0.75 $\pm$ 0.02 & 0.92 $\pm$ 0.00 &  & 0.92 $\pm$ 0.00 \\ 
energydata-complete & 0.81 $\pm$ 0.00 & $\triangleright$ & \bftab 0.78 $\pm$ 0.00 & 0.80 $\pm$ 0.00 & $\triangleright$ & \bftab 0.77 $\pm$ 0.00 & 0.77 $\pm$ 0.00 & $\triangleright$ & \bftab 0.76 $\pm$ 0.00 & 0.77 $\pm$ 0.00 & $\triangleright$ & \bftab 0.74 $\pm$ 0.00 \\ 
FriedmanArtificialDomain & 0.32 $\pm$ 0.00 & $\triangleright$ & \bftab 0.32 $\pm$ 0.00 & 0.33 $\pm$ 0.00 & $\triangleright$ & \bftab 0.32 $\pm$ 0.00 & 0.31 $\pm$ 0.00 &  & \bftab 0.30 $\pm$ 0.00 & 0.60 $\pm$ 0.00 &  & 0.60 $\pm$ 0.00 \\ 
california & \bftab 0.58 $\pm$ 0.00 & $\triangleleft$ & 0.58 $\pm$ 0.00 & \bftab 0.56 $\pm$ 0.00 &  & 0.56 $\pm$ 0.00 & \bftab 0.60 $\pm$ 0.00 &  & 0.60 $\pm$ 0.00 & \bftab 0.54 $\pm$ 0.00 &  & 0.54 $\pm$ 0.00 \\ 
bike & \bftab 0.86 $\pm$ 0.00 &  & 0.90 $\pm$ 0.00 & 0.76 $\pm$ 0.00 &  & \bftab 0.76 $\pm$ 0.00 & \bftab 0.75 $\pm$ 0.00 & $\triangleleft$ & 0.78 $\pm$ 0.00 & 0.70 $\pm$ 0.00 & $\triangleright$ & \bftab 0.68 $\pm$ 0.00 \\ 
3d-spatial-network & 0.60 $\pm$ 0.00 & $\triangleright$ & \bftab 0.57 $\pm$ 0.00 & 0.58 $\pm$ 0.00 & $\triangleright$ & \bftab 0.54 $\pm$ 0.00 & 0.63 $\pm$ 0.00 & $\triangleright$ & \bftab 0.62 $\pm$ 0.00 & 0.60 $\pm$ 0.00 & $\triangleright$ & \bftab 0.56 $\pm$ 0.00 \\ 
Range-Queries-Aggregates & 0.91 $\pm$ 0.00 &  & \bftab 0.91 $\pm$ 0.00 & 0.91 $\pm$ 0.00 & $\triangleright$ & \bftab 0.90 $\pm$ 0.00 & \bftab 0.89 $\pm$ 0.00 &  & 0.89 $\pm$ 0.00 & \bftab 0.86 $\pm$ 0.00 &  & 0.86 $\pm$ 0.00 \\ 
pp-gas-emission & 0.56 $\pm$ 0.00 & $\triangleright$ & \bftab 0.54 $\pm$ 0.00 & 0.56 $\pm$ 0.00 & $\triangleright$ & \bftab 0.54 $\pm$ 0.00 & 0.50 $\pm$ 0.00 &  & \bftab 0.50 $\pm$ 0.00 & 0.70 $\pm$ 0.00 & $\triangleright$ & \bftab 0.68 $\pm$ 0.00 \\ 
GPU-Kernel-Performance & \bftab 0.80 $\pm$ 0.00 & $\triangleleft$ & 0.87 $\pm$ 0.00 & 0.77 $\pm$ 0.00 & $\triangleright$ & \bftab 0.74 $\pm$ 0.00 & 0.68 $\pm$ 0.00 & $\triangleright$ & \bftab 0.55 $\pm$ 0.00 & 0.79 $\pm$ 0.00 & $\triangleright$ & \bftab 0.75 $\pm$ 0.00 \\ 
polution & 0.69 $\pm$ 0.00 & $\triangleright$ & \bftab 0.68 $\pm$ 0.00 & 0.68 $\pm$ 0.00 & $\triangleright$ & \bftab 0.66 $\pm$ 0.00 & 0.69 $\pm$ 0.00 & $\triangleright$ & \bftab 0.68 $\pm$ 0.00 & 0.65 $\pm$ 0.00 & $\triangleright$ & \bftab 0.63 $\pm$ 0.00


==> Tables/sera_Under.tex <==
puma32H & 0.550 $\pm$ 0.001 & $\triangleright$ & \bftab 0.469 $\pm$ 0.001 & 0.644 $\pm$ 0.000 & $\triangleright$ & \bftab 0.527 $\pm$ 0.000 & 0.472 $\pm$ 0.002 & $\triangleright$ & \bftab 0.408 $\pm$ 0.001 & 0.750 $\pm$ 0.000 &  & 0.750 $\pm$ 0.000 \\ 
cpusum & 0.460 $\pm$ 0.001 & $\triangleright$ & \bftab 0.282 $\pm$ 0.000 & \bftab 0.317 $\pm$ 0.000 & $\triangleleft$ & 0.371 $\pm$ 0.003 & 0.473 $\pm$ 0.000 &  & \bftab 0.445 $\pm$ 0.001 & 0.356 $\pm$ 0.000 & $\triangleright$ & \bftab 0.261 $\pm$ 0.000 \\ 
mv & \bftab 0.508 $\pm$ 0.001 &  & 0.514 $\pm$ 0.001 & 0.520 $\pm$ 0.000 & $\triangleright$ & \bftab 0.457 $\pm$ 0.000 & 0.760 $\pm$ 0.002 &  & \bftab 0.750 $\pm$ 0.000 & 0.747 $\pm$ 0.000 & $\triangleright$ & \bftab 0.538 $\pm$ 0.000 \\ 
elevator & 0.887 $\pm$ 0.011 & $\triangleright$ & \bftab 0.775 $\pm$ 0.037 & 0.945 $\pm$ 0.002 & $\triangleright$ & \bftab 0.845 $\pm$ 0.024 & 0.815 $\pm$ 0.006 & $\triangleright$ & \bftab 0.547 $\pm$ 0.000 & 0.921 $\pm$ 0.000 & $\triangleright$ & \bftab 0.385 $\pm$ 0.000 \\ 
energydata-complete & 0.918 $\pm$ 0.000 & $\triangleright$ & \bftab 0.608 $\pm$ 0.000 & 0.906 $\pm$ 0.000 & $\triangleright$ & \bftab 0.616 $\pm$ 0.000 & 0.877 $\pm$ 0.000 & $\triangleright$ & \bftab 0.628 $\pm$ 0.000 & 0.903 $\pm$ 0.000 & $\triangleright$ & \bftab 0.544 $\pm$ 0.001 \\ 
FriedmanArtificialDomain & 0.359 $\pm$ 0.000 & $\triangleright$ & \bftab 0.281 $\pm$ 0.000 & 0.366 $\pm$ 0.000 & $\triangleright$ & \bftab 0.292 $\pm$ 0.000 & 0.340 $\pm$ 0.000 & $\triangleright$ & \bftab 0.259 $\pm$ 0.000 & 0.601 $\pm$ 0.000 &  & 0.601 $\pm$ 0.000 \\ 
california & \bftab 0.584 $\pm$ 0.000 & $\triangleleft$ & 0.608 $\pm$ 0.000 & \bftab 0.556 $\pm$ 0.000 & $\triangleleft$ & 0.580 $\pm$ 0.000 & \bftab 0.591 $\pm$ 0.000 & $\triangleleft$ & 0.614 $\pm$ 0.000 & \bftab 0.532 $\pm$ 0.000 & $\triangleleft$ & 0.555 $\pm$ 0.000 \\ 
bike & 0.891 $\pm$ 0.001 & $\triangleright$ & \bftab 0.786 $\pm$ 0.002 & 0.770 $\pm$ 0.000 & $\triangleright$ & \bftab 0.762 $\pm$ 0.000 & 0.769 $\pm$ 0.000 & $\triangleright$ & \bftab 0.723 $\pm$ 0.000 & 0.797 $\pm$ 0.000 & $\triangleright$ & \bftab 0.589 $\pm$ 0.000 \\ 
3d-spatial-network & 0.675 $\pm$ 0.000 & $\triangleright$ & \bftab 0.484 $\pm$ 0.000 & 0.679 $\pm$ 0.000 & $\triangleright$ & \bftab 0.408 $\pm$ 0.000 & 0.675 $\pm$ 0.000 & $\triangleright$ & \bftab 0.557 $\pm$ 0.000 & 0.696 $\pm$ 0.000 & $\triangleright$ & \bftab 0.421 $\pm$ 0.000 \\ 
Range-Queries-Aggregates & 0.921 $\pm$ 0.000 & $\triangleright$ & \bftab 0.869 $\pm$ 0.000 & 0.914 $\pm$ 0.000 & $\triangleright$ & \bftab 0.860 $\pm$ 0.000 & 0.898 $\pm$ 0.000 & $\triangleright$ & \bftab 0.842 $\pm$ 0.000 & 0.868 $\pm$ 0.000 & $\triangleright$ & \bftab 0.864 $\pm$ 0.000 \\ 
pp-gas-emission & 0.603 $\pm$ 0.000 & $\triangleright$ & \bftab 0.502 $\pm$ 0.000 & 0.626 $\pm$ 0.000 & $\triangleright$ & \bftab 0.477 $\pm$ 0.000 & 0.562 $\pm$ 0.000 & $\triangleright$ & \bftab 0.429 $\pm$ 0.000 & 0.735 $\pm$ 0.000 & $\triangleright$ & \bftab 0.650 $\pm$ 0.000 \\ 
GPU-Kernel-Performance & 0.858 $\pm$ 0.000 & $\triangleright$ & \bftab 0.636 $\pm$ 0.001 & 0.815 $\pm$ 0.000 & $\triangleright$ & \bftab 0.545 $\pm$ 0.000 & 0.744 $\pm$ 0.002 & $\triangleright$ & \bftab 0.585 $\pm$ 0.001 & 0.880 $\pm$ 0.000 & $\triangleright$ & \bftab 0.381 $\pm$ 0.000 \\ 
polution & 0.774 $\pm$ 0.000 & $\triangleright$ & \bftab 0.556 $\pm$ 0.000 & 0.770 $\pm$ 0.000 & $\triangleright$ & \bftab 0.546 $\pm$ 0.000 & 0.761 $\pm$ 0.000 & $\triangleright$ & \bftab 0.574 $\pm$ 0.000 & 0.772 $\pm$ 0.000 & $\triangleright$ & \bftab 0.458 $\pm$ 0.000


==> Tables/tab_datasets_part1_new.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[t]
    \centering
    \caption{Data sets characteristics: number of cases (\#cases) and number of rare cases (\#rare cases) with $thr_\phi=0.8$ that are low extremes (i.e., below the median), high extremes (i.e., above the median), or both.}
    \label{tab1}
    \begin{tabular}{| l | r | r | r | r |}
    \hline
    \multirow{2}{*}{Data set} &
    \multirow{2}{*}{\#cases} & 
    \multicolumn{3}{c|}{\#rare cases ($thr_\phi = 0.8$)} \\
    \cline{3-5}
    & & Low extremes & High extremes & Both extremes \\
    \hline
    puma32H & 8,192 & 422 (5.15\%) & 435 (5.31\%) & 857 (10.46\%) \\ \hline
    cpusum & 8,192 & 722 (8.82\%) & 849 (10.36\%) & 1,571 (19.18\%) \\ \hline
    elevator & 16,599 & 169 (1.02\%) & 2,266 (13.65\%) & 2,435 (14.67\%) \\ \hline
    bike & 17,389 & 4,433 (25.49\%) & 1,301 (7.48\%) & 5,734 (32.97\%) \\ \hline
    energy & 19,735 & 352 (1.78\%) & 2,665 (13.50\%) & 3,017 (15.28\%) \\ \hline
    calhousing & 20,640 & 816 (3.95\%) & 1,821 (8.82\%) & 2,637 (12.77\%) \\ \hline
    gasemission & 36,733 & 199 (0.54\%) & 1,967 (5.36\%) & 2,166 (5.90\%) \\ \hline
    mv & 40,768 & 1,414 (3.47\%) & 9,037 (22.17\%) & 10,451 (25.64\%) \\ \hline
    fried & 40,768 & 739 (1.81\%) & 747 (1.83\%) & 1,486 (3.64\%) \\ \hline
    pollution & 41,757 & 7,462 (17.86\%) & 3,663 (8.77\%) & 11,125 (26.63\%) \\ \hline
    car price & 122,144 & 19,205 (15.72\%) & 14,156 (11.59\%) & 33,361 (27.31\%) \\ \hline
    query & 199,843 & 5,616 (2.81\%) & 3,115 (1.56\%) & 8,731 (4.37\%) \\ \hline
    GPU & 241,600 & 18,033 (7.46\%) & 36,493 (15.10\%) & 54,526 (22.56\%) \\ \hline
    3d & 434,873 & 30 (0.01\%) & 30,718 (7.06\%) & 30,748 (7.07\%) \\ \hline
    \end{tabular}
\end{table}

==> Tables/tab_datasets_part2_new.tex <==
\begin{table}[h]
    \centering
    \caption{Data Set Characteristics}\label{tab_datasets_part2}
    \begin{tabular}{|l|l|l|l|}
        \hline
        Data set & Data Set Full Name & \#Attributes & \#Examples \\ \hline
        puma32H\tablefootnote[1]{\url{https://sci2s.ugr.es/keel/datasets.php}} & Pumadyn & 32 & 8,192 \\ \hline
        cpusum\tablefootnote[2]{\url{https://www.dcc.fc.up.pt/~ltorgo/Regression/DataSets.html}} & Computer Activity & 21 & 8,192 \\ \hline
        elevator\textsuperscript{1} & Elevators & 18 & 16,599 \\ \hline
        bike\tablefootnote[3]{\url{https://archive.ics.uci.edu/ml/datasets.php}} & Bike Sharing & 16 & 17,379 \\ \hline
        energy\textsuperscript{3} & Appliances Energy Prediction & 29 & 19,735 \\ \hline
        calhousing\textsuperscript{1} & California Housing & 8 & 20,639 \\ \hline
        gasemission\textsuperscript{3} & Gas Turbine CO and NOx Emission & 11 & 36,733 \\ \hline
        mv\textsuperscript{2} & MV Artificial Domain & 10 & 40,768 \\ \hline
        fried\textsuperscript{2} & Friedman Artificial Domain & 10 & 40,768 \\ \hline
        pollution\textsuperscript{3} & Beijing PM2.5 Data & 13 & 41,757 \\ \hline
        car price\tablefootnote[4]{\url{https://www.kaggle.com/tsaustin/us-used-car-sales-data}} & US Used Car Sales Data & 12 & 122,144 \\ \hline
        query\textsuperscript{3} & Query Analytics Workloads & 8 & 199,843 \\ \hline
        GPU\textsuperscript{3} & SGEMM GPU Kernel Performance & 18 & 241,600 \\ \hline
        3d\textsuperscript{3} & 3D Road Network & 4 & 434,873 \\ \hline
    \end{tabular}
\end{table}

==> Tables/tab_datasets_part3_new.tex <==
\setlength{\tabcolsep}{2pt}
\begin{table}[t]
    \centering
    \caption{Data sets characteristics: number of cases (\#cases) and number of rare cases (\#rare cases) with $thr_\phi=0.9$ that are low extremes (i.e., below the median), high extremes (i.e., above the median), or both.}
    \label{tab_datasets_part3}
    \begin{tabular}{| l | r | r | r | r |}
    \hline
    \multirow{2}{*}{Data set} &
    \multirow{2}{*}{\#cases} & 
    \multicolumn{3}{c|}{\#rare cases ($thr_\phi = 0.9$)} \\
    \cline{3-5}
    & & Low extremes & High extremes & Both extremes \\
    \hline
        puma32H & 8,192 & 266 (3.25\%)  & 273 (3.33\%)  & 539 (6.58\%)  \\ \hline
        cpusum & 8,192 & 621 (7.58\%)  & 433 (5.29\%)  & 1,054 (12.87\%)  \\ \hline
        elevator & 16,599 & 55 (0.33\%)  & 2,025 (12.20\%)  & 2,080 (12.53\%)  \\ \hline
        bike & 17,379 & 3,623 (20.85\%)  & 981 (5.64\%)  & 4,604 (26.49\%)  \\ \hline
        energy & 19,735 & 9 (0.05\%)  & 2,442 (12.37\%)  & 2,451 (12.42\%)  \\ \hline
        calhousing & 20,639 & 127 (0.62\%)  & 1,515 (7.34\%)  & 1,642 (7.96\%)  \\ \hline
        gasemission & 36,733 & 47 (0.13\%)  & 1,434 (3.90\%)  & 1,481 (4.03\%)  \\ \hline
        mv & 40,768 & 537 (1.32\%)  & 5,108 (12.53\%)  & 5,645 (13.85\%)  \\ \hline
        fried & 40,768 & 278 (0.68\%)  & 313 (0.77\%)  & 591 (1.45\%)  \\ \hline
        polution & 41,757 & 4,467 (10.70\%)  & 2,929 (7.01\%)  & 7,396 (17.71\%)  \\ \hline
        car price & 122,144 & 12,499 (10.23\%)  & 11,849 (9.70\%)  & 24,348 (19.93\%)  \\ \hline
        query & 199,843 & 3,084 (1.54\%)  & 1,356 (0.68\%)  & 4,440 (2.22\%)  \\ \hline
        GPU & 241,600 & 8,014 (3.32\%)  & 36,065 (14.93\%)  & 44,079 (18.25\%)  \\ \hline
        3d & 434,873 & 3 (0.00\%)  & 23,182 (5.33\%)  & 23,185 (5.33\%)  \\ \hline
    \end{tabular}
\end{table}

==> Tables/tab_datasets_part4_new.tex <==
\setlength{\tabcolsep}{2pt}
    \begin{table}[t]
    \centering
    \caption{Data sets characteristics: number of cases (\#cases) and number of rare cases (\#rare cases) with $thr_\phi=1.0$ that are low extremes (i.e., below the median), high extremes (i.e., above the median), or both.}
    \label{tab_datasets_part4}
    \begin{tabular}{| l | r | r | r | r |}
    \hline
    \multirow{2}{*}{Data set} &
    \multirow{2}{*}{\#cases} & 
    \multicolumn{3}{c|}{\#rare cases ($thr_\phi = 1.0$)} \\
    \cline{3-5}
    & & Low extremes & High extremes & Both extremes \\
    \hline
        puma32H & 8,192 & 57 (0.7\%) & 68 (0.83\%) & 125 (1.52\%) \\ \hline
        cpusum & 8,192 & 469 (5.73\%) & 61 (0.74\%) & 530 (6.47\%) \\ \hline
        elevator & 16,599 & 13 (0.08\%) & 1,762 (10.62\%) & 1,775 (10.70\%) \\ \hline
        bike & 17,379 & 158 (0.91\%) & 509 (2.93\%) & 667 (3.84\%) \\ \hline
        energy & 19,735 & 9 (0.05\%) & 2,208 (11.19\%) & 2,217 (11.24\%) \\ \hline
        calhousing & 20,639 & 4 (0.02\%) & 1,072 (5.19\%) & 1,076 (5.21\%) \\ \hline
        gasemission & 36,733 & 5 (0.01\%) & 933 (2.54\%) & 938 (2.55\%) \\ \hline
        mv & 40,768 & 2 (0.00\%) & 1 (0.00\%) & 3 (0.00\%) \\ \hline
        fried & 40,768 & 7 (0.02\%) & 20 (0.05\%) & 27 (0.07\%) \\ \hline
        polution & 41,757 & 2 (0.00\%) & 1,797 (4.30\%) & 1,799 (4.30\%) \\ \hline
        car price & 122,144 & 31 (0.03\%) & 8,405 (6.88\%) & 8,436 (6.91\%) \\ \hline
        query & 199,843 & 868 (0.43\%) & 147 (0.07\%) & 1,015 (0.50\%) \\ \hline
        GPU & 241,600 & 1 (0.00\%) & 26,857 (11.12\%) & 26,858 (11.12\%) \\ \hline
        3d & 434,873 & 1 (0.00\%) & 11,666 (2.68\%) & 11,667 (2.68\%) \\ \hline
    \end{tabular}
\end{table}

==> Tables/tables-phi.tex <==
% ====================   Double-side ================
        % == Both sides OS RMSE_PHI_0.0
        \begin{table}[!h]
            \centering
            \caption{$RMSE$ and $RMSE_{\phi}$ estimates considering all the observations: $thr_\phi = 0$.} \label{tab:estimates_Both_OS_RMSE_PHI_ALL}
            \resizebox{\textwidth}{!}{
                \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
                \hline
                \multicolumn{13}{|c|}{$RMSE_{\phi}$ estimates for the {\tt chebyOS} method.}\\
                \hline
                \multirow{2}{4em}{data set}&
                \multicolumn{3}{|c|}{Perceptron} & 
                \multicolumn{3}{|c|}{FIMT-DD} & 
                \multicolumn{3}{|c|}{TargetMean}&
                \multicolumn{3}{|c|}{AMRules}
                \\
                 \cline{2-13}&
                 \multicolumn{1}{|c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & 
                \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} \\
                \hline 
                \input{Tables/both_OS_phi_0_}
                {\bf Avg. Rank} & 
                \multicolumn{1}{|c|}{ 4.79 }  & \multicolumn{2}{|c|}{ 3.0 }  & \multicolumn{1}{|c|}{ 3.64 }  & \multicolumn{2}{|c|}{ 2.07 }  & \multicolumn{1}{|c|}{ 6.07 }  & \multicolumn{2}{|c|}{ 4.43 }  & \multicolumn{1}{|c|}{ 6.57 }  & \multicolumn{2}{|c|}{ 5.43 } \\
                \hline
                \end{tabular}
            }
        
%         % == Both sides US RMSE_PHI_0.0
                \resizebox{\textwidth}{!}{
                \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
                \hline
                \multicolumn{13}{|c|}{$RMSE_{\phi}$ estimates for the {\tt chebyUS} method.}\\
                \hline
                \multirow{2}{4em}{data set}&
                \multicolumn{3}{|c|}{Perceptron} & 
                \multicolumn{3}{|c|}{FIMT-DD} & 
                \multicolumn{3}{|c|}{TargetMean}&
                \multicolumn{3}{|c|}{AMRules}
                \\
                 \cline{2-13}&
                 \multicolumn{1}{|c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & 
                \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} \\
                \hline
                \input{Tables/both_US_phi_0_}
                {\bf Avg. Rank} & 
                \multicolumn{1}{|c|}{4.68} & 
                \multicolumn{2}{|c|}{2.25} & 
                \multicolumn{1}{c|}{3.68} & 
                \multicolumn{2}{|c|}{2.68} & 
                \multicolumn{1}{c|}{5.82} & 
                \multicolumn{2}{|c|}{4.96} & 
                \multicolumn{1}{c|}{6.32} & 
                \multicolumn{2}{|c|}{5.61} \\
                \hline
                \end{tabular}
                }




%         % == Both sides OS RMSE_NORMAL_0.0
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
            \hline
            \multicolumn{13}{|c|}{$RMSE$ estimate for the {\tt chebyOS} method.}\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
              \cline{2-13}&
             \multicolumn{1}{|c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & 
            \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} \\
            \hline
            \input{Tables/both_OS_normal_0_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 4.93 }  & \multicolumn{2}{|c|}{ 3.04 }  & \multicolumn{1}{|c|}{ 3.61 }  & \multicolumn{2}{|c|}{ 2.0 }  & \multicolumn{1}{|c|}{ 6.04 }  & \multicolumn{2}{|c|}{ 4.46 }  & \multicolumn{1}{|c|}{ 6.54 }  & \multicolumn{2}{|c|}{ 5.39 } \\
            \hline
            \end{tabular}
            }
            
%         % == Both sides US RMSE_NORMAL_0.0
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
            \hline
            \multicolumn{13}{|c|}{$RMSE$ estimate for the {\tt chebyUS} method.}\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
             \cline{2-13}
            & \multicolumn{1}{|c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & 
            \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} \\
            \hline
            \input{Tables/both_US_normal_0_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{4.68} & 
            \multicolumn{2}{|c|}{2.25} & 
            \multicolumn{1}{c|}{3.68} & 
            \multicolumn{2}{|c|}{2.68} & 
            \multicolumn{1}{c|}{5.82} & 
            \multicolumn{2}{|c|}{4.96} & 
            \multicolumn{1}{c|}{6.32} & 
            \multicolumn{2}{|c|}{5.61} \\
            \hline
            \end{tabular}
            }
            \end{table}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


    
%         % == Both sides OS RMSE_PHI_0.8  =Done
        \begin{table}[!h]
            \centering
            \caption{$RMSE$ and $RMSE_{\phi}$ estimates considering {\tt all} (double-side) rare cases: $thr_\phi = 0.8$.} \label{tab:estimates_Both_OS_RMSE_PHI_08}
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
            \hline
            \multicolumn{13}{|c|}{$RMSE_{\phi}$ estimate for the {\tt chebyOS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
            \cline{2-13}&
             \multicolumn{1}{|c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & 
            \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} \\
            \hline
            \input{Tables/both_OS_Phi_8_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 4.79 }  & \multicolumn{2}{|c|}{ 3.0 }  & \multicolumn{1}{|c|}{ 3.64 }  & \multicolumn{2}{|c|}{ 2.07 }  & \multicolumn{1}{|c|}{ 6.07 }  & \multicolumn{2}{|c|}{ 4.43 }  & \multicolumn{1}{|c|}{ 6.57 }  & \multicolumn{2}{|c|}{ 5.43 } \\
            \hline
            \end{tabular}
            }
           % \end{table}
            
%         % == Both sides US RMSE_PHI_0.8 =Done
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
             \hline
            \multicolumn{13}{|c|}{$RMSE_{\phi}$ estimate for the {\tt chebyUS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
             \cline{2-13}
            & \multicolumn{1}{|c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & 
            \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} \\
            \hline
            \input{Tables/both_US_Phi_8_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 4.68 }  & \multicolumn{2}{|c|}{ 2.25 }  & \multicolumn{1}{|c|}{ 3.68 }  & \multicolumn{2}{|c|}{ 2.68 }  & \multicolumn{1}{|c|}{ 5.82 }  & \multicolumn{2}{|c|}{ 4.96 }  & \multicolumn{1}{|c|}{ 6.32 }  & \multicolumn{2}{|c|}{ 5.61 } \\
            \hline
            \end{tabular}
            }
            
            
%         % == Both sides OS RMSE_NORMAL_0.8 =Done
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
             \hline
            \multicolumn{13}{|c|}{$RMSE$ estimate for the {\tt chebyOS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
             \cline{2-13}&
             \multicolumn{1}{|c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & 
            \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} \\
            \hline            
                \input{Tables/both_OS_normal_8_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 4.93 }  & \multicolumn{2}{|c|}{ 3.04 }  & \multicolumn{1}{|c|}{ 3.61 }  & \multicolumn{2}{|c|}{ 2.0 }  & \multicolumn{1}{|c|}{ 6.04 }  & \multicolumn{2}{|c|}{ 4.46 }  & \multicolumn{1}{|c|}{ 6.54 }  & \multicolumn{2}{|c|}{ 5.39 } \\

            \hline
            \end{tabular}
            }
            
%         % == Both sides US RMSE_NORMAL_0.8 =Done

            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
            \hline
             \multicolumn{13}{|c|}{$RMSE$ estimate for the {\tt chebyUS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
             \cline{2-13}
            & \multicolumn{1}{|c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & 
            \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} \\
            \hline
            \input{Tables/both_US_normal_8_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 4.71 }  & \multicolumn{2}{|c|}{ 2.5 }  & \multicolumn{1}{|c|}{ 3.5 }  & \multicolumn{2}{|c|}{ 2.86 }  & \multicolumn{1}{|c|}{ 5.64 }  & \multicolumn{2}{|c|}{ 5.14 }  & \multicolumn{1}{|c|}{ 6.14 }  & \multicolumn{2}{|c|}{ 5.5 } \\

            \hline
            \end{tabular}
            }
            \end{table}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%         % == Both sides OS RMSE_PHI_0.9 = Done
        \begin{table}[!h]
            \centering
            \caption{$RMSE$ and $RMSE_{\phi}$ estimates considering {\tt all} (double-side) rare cases: $thr_\phi = 0.9$.} \label{tab:estimates_Both_OS_RMSE_PHI_09}
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
            \hline
            \multicolumn{13}{|c|}{$RMSE_{\phi}$ estimate for the {\tt chebyOS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
            \cline{2-13}&
             \multicolumn{1}{|c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & 
            \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} \\
            \hline
            \input{Tables/both_OS_Phi_9_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 5.14 }  & \multicolumn{2}{|c|}{ 2.82 }  & \multicolumn{1}{|c|}{ 3.68 }  & \multicolumn{2}{|c|}{ 2.07 }  & \multicolumn{1}{|c|}{ 5.93 }  & \multicolumn{2}{|c|}{ 4.32 }  & \multicolumn{1}{|c|}{ 6.71 }  & \multicolumn{2}{|c|}{ 5.32 } \\
            \hline
            \end{tabular}
            }

            
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
               \hline
            \multicolumn{13}{|c|}{$RMSE_{\phi}$ estimate for the {\tt chebyUS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
             \cline{2-13}
            & \multicolumn{1}{|c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & 
            \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} \\
            \hline
            \input{Tables/both_US_Phi_9_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 5.07 }  & \multicolumn{2}{|c|}{ 2.29 }  & \multicolumn{1}{|c|}{ 3.71 }  & \multicolumn{2}{|c|}{ 2.71 }  & \multicolumn{1}{|c|}{ 5.79 }  & \multicolumn{2}{|c|}{ 4.68 }  & \multicolumn{1}{|c|}{ 6.5 }  & \multicolumn{2}{|c|}{ 5.25 } \\
            \hline
            \end{tabular}
            }


            
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
            \hline
            \multicolumn{13}{|c|}{$RMSE$ estimate for the {\tt chebyOS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
            \cline{2-13}&
             \multicolumn{1}{|c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & 
            \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} \\
            \hline            
            \input{Tables/both_OS_normal_9_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 5.14 }  & \multicolumn{2}{|c|}{ 2.79 }  & \multicolumn{1}{|c|}{ 3.64 }  & \multicolumn{2}{|c|}{ 2.21 }  & \multicolumn{1}{|c|}{ 5.93 }  & \multicolumn{2}{|c|}{ 4.29 }  & \multicolumn{1}{|c|}{ 6.71 }  & \multicolumn{2}{|c|}{ 5.29 } \\

            \hline
            \end{tabular}
            }

            
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
             \hline
            \multicolumn{13}{|c|}{$RMSE$ estimate for the {\tt chebyUS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
             \cline{2-13}
            & \multicolumn{1}{|c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & 
            \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} \\
            \hline            
            \input{Tables/both_US_normal_9_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 5.0 }  & \multicolumn{2}{|c|}{ 2.39 }  & \multicolumn{1}{|c|}{ 3.43 }  & \multicolumn{2}{|c|}{ 2.75 }  & \multicolumn{1}{|c|}{ 5.71 }  & \multicolumn{2}{|c|}{ 4.89 }  & \multicolumn{1}{|c|}{ 6.43 }  & \multicolumn{2}{|c|}{ 5.39 } \\
            \hline
            \end{tabular}
            }
            \end{table}



% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%         % == Both sides OS RMSE_PHI_1.0 = Done
        \begin{table}[!h]
            \centering
            \caption{$RMSE$ and $RMSE_{\phi}$ estimates considering {\tt all} (double-side) rare cases: $thr_\phi = 1.0$.} \label{tab:estimates_Both_OS_RMSE_PHI_10}
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
             \hline
            \multicolumn{13}{|c|}{$RMSE_{\phi}$ estimate for the {\tt chebyOS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
             \cline{2-13}&
             \multicolumn{1}{|c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & 
            \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} \\
            \hline
                \input{Tables/both_OS_Phi_1_}
            \hline
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 5.07 }  & \multicolumn{2}{|c|}{ 2.93 }  & \multicolumn{1}{|c|}{ 3.93 }  & \multicolumn{2}{|c|}{ 1.86 }  & \multicolumn{1}{|c|}{ 6.11 }  & \multicolumn{2}{|c|}{ 4.14 }  & \multicolumn{1}{|c|}{ 6.86 }  & \multicolumn{2}{|c|}{ 5.11 } \\
            \hline
            \end{tabular}
            }

            
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
            \hline
            \multicolumn{13}{|c|}{$RMSE_{\phi}$ estimate for the {\tt chebyUS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
             \cline{2-13}
            & \multicolumn{1}{|c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & 
            \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} \\
            \hline            
            \input{Tables/both_US_Phi_1_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 5.11 }  & \multicolumn{2}{|c|}{ 2.32 }  & \multicolumn{1}{|c|}{ 3.96 }  & \multicolumn{2}{|c|}{ 2.32 }  & \multicolumn{1}{|c|}{ 6.25 }  & \multicolumn{2}{|c|}{ 4.32 }  & \multicolumn{1}{|c|}{ 6.89 }  & \multicolumn{2}{|c|}{ 4.82 } \\
            \hline
            \end{tabular}
            }

            
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
             \hline
            \multicolumn{13}{|c|}{$RMSE$ estimate for the {\tt chebyOS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
             \cline{2-13}&
             \multicolumn{1}{|c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & 
            \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} \\
            \hline            
            \input{Tables/both_OS_normal_1_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 5.07 }  & \multicolumn{2}{|c|}{ 2.93 }  & \multicolumn{1}{|c|}{ 3.93 }  & \multicolumn{2}{|c|}{ 1.86 }  & \multicolumn{1}{|c|}{ 6.11 }  & \multicolumn{2}{|c|}{ 4.14 }  & \multicolumn{1}{|c|}{ 6.86 }  & \multicolumn{2}{|c|}{ 5.11 } \\
            \hline
            \end{tabular}
            }
            
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
             \hline
            \multicolumn{13}{|c|}{$RMSE$ estimate for the {\tt chebyUS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
             \cline{2-13}
            & \multicolumn{1}{|c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & 
            \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} \\
            \hline
            \input{Tables/both_US_normal_1_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 5.11 }  & \multicolumn{2}{|c|}{ 2.32 }  & \multicolumn{1}{|c|}{ 3.96 }  & \multicolumn{2}{|c|}{ 2.32 }  & \multicolumn{1}{|c|}{ 6.25 }  & \multicolumn{2}{|c|}{ 4.32 }  & \multicolumn{1}{|c|}{ 6.89 }  & \multicolumn{2}{|c|}{ 4.82 } \\
            \hline
            \end{tabular}
            }
            \end{table}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % ====================   One-side ================

%         % == LEFT sides OS RMSE_PHI_0.8 =Done
        \begin{table}[!h]
            \centering
            \caption{$RMSE_{\phi}$ estimates considering {\tt left-hand side} rare cases ($thr_\phi = 0.8$).} \label{tab:estimates_LEFT_OS_RMSE_PHI_08}
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
             \hline
            \multicolumn{13}{|c|}{$RMSE_{\phi}$ estimate for the {\tt chebyOS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
             \cline{2-13}&
             \multicolumn{1}{|c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & 
            \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} \\
            \hline            
            \input{Tables/left_OS_phi_8_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 5.54 }  & \multicolumn{2}{|c|}{ 2.64 }  & \multicolumn{1}{|c|}{ 4.71 }  & \multicolumn{2}{|c|}{ 1.89 }  & \multicolumn{1}{|c|}{ 6.68 }  & \multicolumn{2}{|c|}{ 3.25 }  & \multicolumn{1}{|c|}{ 7.39 }  & \multicolumn{2}{|c|}{ 3.89 } \\
            \hline
            \end{tabular}
            }
            
        % == LEFT sides US RMSE_PHI_0.8 = Done
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
            \hline
            \multicolumn{13}{|c|}{$RMSE_{\phi}$ estimate for the {\tt chebyUS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
             \cline{2-13}
            & \multicolumn{1}{|c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & 
            \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} \\
            \hline                      
            \input{Tables/left_US_phi_8_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 5.11 }  & \multicolumn{2}{|c|}{ 2.29 }  & \multicolumn{1}{|c|}{ 4.32 }  & \multicolumn{2}{|c|}{ 3.39 }  & \multicolumn{1}{|c|}{ 6.32 }  & \multicolumn{2}{|c|}{ 3.96 }  & \multicolumn{1}{|c|}{ 7.04 }  & \multicolumn{2}{|c|}{ 3.57 } \\
            \hline
            \end{tabular}
            }
            \end{table}


        % == RIGHT sides OS RMSE_PHI_0.8 = Done
        \begin{table}[!h]
            \centering
            \caption{$RMSE_{\phi}$ estimates
            considering {\tt right-hand side} rare cases ($thr_\phi = 0.8$).} \label{tab:estimates_RIGHT_OS_RMSE_PHI_08}
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
            \hline
            \multicolumn{13}{|c|}{$RMSE_{\phi}$ estimate for the {\tt chebyOS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
            \cline{2-13}&
             \multicolumn{1}{|c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} & 
            \multicolumn{1}{c|}{Baseline} & \multicolumn{2}{|c|}{ChebyOS} \\
            \hline          
            \input{Tables/right_OS_phi_8_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 6.07 }  & \multicolumn{2}{|c|}{ 2.25 }  & \multicolumn{1}{|c|}{ 4.89 }  & \multicolumn{2}{|c|}{ 1.71 }  & \multicolumn{1}{|c|}{ 6.57 }  & \multicolumn{2}{|c|}{ 3.64 }  & \multicolumn{1}{|c|}{ 6.86 }  & \multicolumn{2}{|c|}{ 4.0 } \\
            \hline
            \end{tabular}
            }
            
        % == RIGHT sides US RMSE_PHI_0.8 = Done
            \resizebox{\textwidth}{!}{
            \begin{tabular}{ |l|r|rr|r|rr|r|rr|r|rr|}
            \hline
            \multicolumn{13}{|c|}{$RMSE_{\phi}$ estimate for the {\tt chebyUS} method. }\\
            \hline
            \multirow{2}{4em}{data set}&
            \multicolumn{3}{|c|}{Perceptron} & 
            \multicolumn{3}{|c|}{FIMT-DD} & 
            \multicolumn{3}{|c|}{TargetMean}&
            \multicolumn{3}{|c|}{AMRules}
            \\
             \cline{2-13}
            & \multicolumn{1}{|c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} & 
            \multicolumn{1}{c|}{Baseline} & 
            \multicolumn{2}{|c|}{ChebyUS} \\
            \hline          
            \input{Tables/right_US_phi_8_}
            {\bf Avg. Rank} & 
            \multicolumn{1}{|c|}{ 6.07 }  & \multicolumn{2}{|c|}{ 2.61 }  & \multicolumn{1}{|c|}{ 4.89 }  & \multicolumn{2}{|c|}{ 2.57 }  & \multicolumn{1}{|c|}{ 6.5 }  & \multicolumn{2}{|c|}{ 3.11 }  & \multicolumn{1}{|c|}{ 6.82 }  & \multicolumn{2}{|c|}{ 3.43 } \\
            \hline
            \end{tabular}
            }
            \end{table}


